Min-CSPs on Complete Instances

Given a fixed arity $k \geq 2$, Min-$k$-CSP on complete instances involves a set of $n$ variables $V$ and one nontrivial constraint for every $k$-subset of variables (so there are $\binom{n}{k}$ constraints). The goal is to find an assignment that minimizes unsatisfied constraints. Unlike Max-$k$-CSP that admits a PTAS on dense or expanding instances, the approximability of Min-$k$-CSP is less understood. For some CSPs like Min-$k$-SAT, there's an approximation-preserving reduction from general to dense instances, making complete instances unique for potential new techniques. This paper initiates a study of Min-$k$-CSPs on complete instances. We present an $O(1)$-approximation algorithm for Min-2-SAT on complete instances, the minimization version of Max-2-SAT. Since $O(1)$-approximation on dense or expanding instances refutes the Unique Games Conjecture, it shows a strict separation between complete and dense/expanding instances. Then we study the decision versions of CSPs, aiming to satisfy all constraints; which is necessary for any nontrivial approximation. Our second main result is a quasi-polynomial time algorithm for every Boolean $k$-CSP on complete instances, including $k$-SAT. We provide additional algorithmic and hardness results for CSPs with larger alphabets, characterizing (arity, alphabet size) pairs that admit a quasi-polynomial time algorithm on complete instances.

==> Inputs/3csp-old-classification.tex <==
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{All Variants of Symmetric \texorpdfstring{$\ncsp{3}$}{error}}
    \aay{We don't even need to define all these variants. It's either \kitwocsp ($O(n^2)$) or \threesat ($n^{O(\log n)}$)}.


    
    In every boolean symmetric \ncsp{3}, we are given a set of $n$ boolean variables $V$, and clauses $\cC$ containing literals of three variables. The instance is called \emph{complete} if for every triplet of variables, there is a clause with their literals in it. Thus, the total number of clauses in a complete instance is \aay{at least} $\binom{n}{3}$.

    In the \Cref{tab:class}, we classify boolean 3CSPs based on the number of true literals required to satisfy a clause. A problem is exactly defined by the non-empty set $S\subseteq [3]$, where a clause is satisfied if and only if the number of true literals in the clause belongs to the set $S$.

    
    For any problem $\cP$ with clauses $\cC$ and predicates $P_C$ for each clause $C\in\cC$, we define $\neg \cP$ as the problem with the set of same clauses $\cC$ but with different predicates $P'_C$ such that $P'_C(\alpha(C)) = P_C(\neg \alpha(C))$ for all assignments $\alpha(C)\in\{0,1\}^{|C|}$.%with clauses $\cC'$ obtained by negating all the literals of every clause in $\cC$. That is, for every clause $(\ell_1, \ell_2, \ell_3)\in \cC$ of $P$ there is a clause $(\neg\ell_1, \neg\ell_2, \neg\ell_3)\in \cC'$. 
    For every satisfying assignment $\alpha(V)$ of $P$, the negated assignment $\neg\alpha(V)$ is satisfying assignment for $\neg P$. \aayr{do we need to define $\neg\alpha(C)$?}

    
    \begin{table}[!htb]
    \caption{All possible 3CSPs.}
    \label{tab:class}
    \begin{center}
    \begin{tabular}{c|c|c}
        Problem &Satisfying $\#$Variables & Decision Algorithm \\\hline
        $\neg$3AND & $\{0\}$&$\poly(n)$ \\
        $\neg\atleasttwo$& $\{0,1\}$ &  $\poly(n)$ (\Cref{thm:induced2csp})\\
        $\neg$3LIN & $\{0,2\}$ & $\poly(n)$\\
        $\allnone$ & $\{0,3\}$ & $\poly(n)$\\
        $\neg\threesat$& $\{0,1,2\}$ & $n^{O(\log n)}$(\Cref{thm:3satassgn})\\
        $\neg\notone$& $\{0,1,3\}$ & $\poly(n)$(\Cref{thm:induced2csp})\\
        $\notone$& $\{0,2,3\}$ & $\poly(n)$(\Cref{thm:induced2csp})\\
        $\onlyone$& $\{1\}$ & $\poly(n)$ (\Cref{thm:induced2csp})\\
        $\nae$& $\{1,2\}$ & $\poly(n)$ (\Cref{thm:induced2csp})\\
        3LIN & $\{1,3\}$ & $\poly(n)$\\
        $\threesat$& $\{1,2,3\}$ & $n^{O(\log n)}$ (\Cref{thm:3satassgn}) \\
        $\neg \onlyone$& $\{2\}$ & $\poly(n)$ (\Cref{thm:induced2csp})\\
        $\atleasttwo$& $\{2,3\}$ & $\poly(n)$ (\Cref{thm:induced2csp})\\
        3AND & $\{3\}$ & $\poly(n)$\\
    \end{tabular}
    \end{center}
    \end{table}

    

    
    % \begin{center}
    % \begin{tabular}{c|c|c}
    %     Problem &Satisfying $\#$Variables & Decision Algorithm \\\hline
    %     $\threesat$ & $\{1,2,3\}$ & $n^{O(\log n)}$(\Cref{alg:3sat})\\
    %     $\nae$ & $\{1,2\}$ & $\poly(n)$(\Cref{thm:naedet}) \\
    %     $\onlyone$ & $\{1\}$ & $\poly(n)$(\Cref{thm:onlyonedet}) \\
    %     $\notone$ & $\{0,2,3\}$ & $n^{O(\log n)}$(\Cref{thm:not1}) \\
    %     $\threelin$ & $\{0,2\}$ & $\poly(n)$ \\
    %     $\threeand$ & $\{3\}$ & $\poly(n)$ \\
    %     $\allnone$ & $\{0,3\}$ & $\poly(n)$
    % \end{tabular}
    % \end{center}


    \paragraph{\texorpdfstring{$\onlyone$}{Only-1} Decision Version.} In the $\onlyone$ problem, we are given $n$ variables $V$, $\binom{n}{3}$ clauses $\cC$ of length $3$ each such that every triplet of variables appear as literals in a clause. A clause is satisfied if and only if exactly one of the literals is assigned $1$, and the other two are assigned $0$. Thus, for every satisfying assignment, a clause would have exactly one literal in the minority. This is similar to $\nae$ where the satisfied clauses have minority variables. In fact, for $\onlyone$ it is even simpler as the minority variable is always assigned the value $1$. Thus, our algorithm for $\nae$ works for $\onlyone$. 

    \paragraph{$\threelin,\ \threeand$ Decision Version.} Both $\threelin,\ \threeand$ have polynomial time decision algorithms.% \aayr{cite results}

    \paragraph{$\allnone$ Decision Version.} In $\allnone$ problem, a clause is satisfied if and only if the literals are set to either all $1$ or all $0$. The algorithm decide whether the input instance is satisfiable or not simply guesses the value of an arbitrary (unfixed) variable $v$, fixes the other variables corresponding to the clauses of $v$, and then recursively solves the problem. Since every variable is in at least $\Omega(n^2)$ clauses out of a total of $\binom{n}{3}$, then fixing the variable fixes at least $\Omega(\frac1n)$ fraction of the clauses. Thus, in algorithm takes $O(n)$ iterations. %The correctness of the algorithm follows simply.

    %\paragraph{$\threeand,\ \allnone$ Decision Version} In the $\threeand$ problem, a clause is satisfied if and only if all the literals are set to true. This can be easily reduced to the decision version of $\twosat$. For every $3$-clause ($\ell_1, \ell_2, \ell_3)$, consider the $2$-clauses: $(\neg \ell_i, \ell_j), (\ell_i, \neg \ell_j)$, for all $i\neq j \in [3]$. A similar idea works for the $\allnone$ problem.
    %Given an instance of $\all$ with variables $V=\{v_i\}_{i\in[n]}$ and clauses $\cC$, construct a graph $G(L=\{l_i\}_{i\in[2n]}, E)$, where the $l_i$ and $l_(n+i)$ correspond to literals $v_i$ and $\neg v_i$ respectively. Add edge $(l_i, l_j), (l_j, l_k)$ for every clause on literals $(\ell_i, \ell_j, \ell_k)$. The problem reduces to deciding whether there is a connected component of the graph with no two literals from the same variable or not in $G$. This can be done in polynomial time. A similar idea works for the $\allnone$ problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


==> Inputs/header_camready.tex <==
% %Useful approx. macros


% \date{\today}

%packages
% \usepackage[letterpaper]{geometry}
% \usepackage[utf8]{inputenc}
% \usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
% \usepackage[hidelinks]{hyperref}
\usepackage{cleveref}
\usepackage{xcolor}
\usepackage{fullpage}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{xspace}
\usepackage{multirow}
\usepackage{diagbox}
\usepackage[colorinlistoftodos,textsize=tiny,textwidth=2cm,color=green!50!gray]{todonotes}

\usepackage{thmtools, thm-restate} %for restate theorems and all

\usepackage{bm}

% \usepackage{silence}

% Filter out all font shape warnings
% \WarningFilter{latexfont}{Font shape `OT1/cmr/bx/sc' undefined}
% \WarningFilter{latexfont}{Font shape}
% \WarningFilter{latexfont}{Some font shapes were not available, defaults substituted.}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}

\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

\usepackage{derivative} % has commands like \pdv{f}{x,y,z} = \del^3 (f)/\del(x)\del(y)\del(z)
\usepackage{mathtools} % for \boxed (normal box) and \Aboxed (box across alignment tabs)
\usepackage{bbm} %\mathbbm{1} := indicator function
\usepackage{tikz}
\usepackage{forest}
%macros
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}{Claim}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{example}[theorem]{Example}
\newtheorem{definition}{Definition}[Definition]
% \let\definition\Definition
% \let\enddefinition\endDefinition


\newtheorem{remark}{Remark}[Remark]
\newtheorem{question}{Question}[section]
\newtheorem{observation}{Observation}[section]
% \newtheorem{openq}{Question}[section]


\crefname{@theorem}{Theorem}{Theorems}
\crefname{claim}{Claim}{Claims}
\crefname{definition}{definition}{Theorems}
\crefname{remark}{Theorem}{Theorems}
\crefname{question}{Theorem}{Theorems}
\crefname{observation}{Theorem}{Theorems}

\Crefname{@theorem}{Theorem}{Theorems}
\Crefname{claim}{Claim}{Claims}
\Crefname{definition}{definition}{Theorems}
\Crefname{remark}{Theorem}{Theorems}
\Crefname{question}{Theorem}{Theorems}
\Crefname{observation}{Theorem}{Theorems}



% \def\DEBUG{true} % comment out this line to remove comments
\ifdefined\DEBUG
    \newcommand{\adi}[1]{\textcolor{red}{#1}}
    \newcommand{\eui}[1]{\textcolor{green}{#1}}
    \newcommand{\aay}[1]{\textcolor{blue}{#1}}
    
    \def\rem#1{{\marginpar{\raggedright\scriptsize #1}}}
    \newcommand{\adir}[1]{\rem{\textcolor{red}{$\bullet$ #1}}}
    \newcommand{\euir}[1]{\rem{\textcolor{green}{$\bullet$ #1}}}
    \newcommand{\aayr}[1]{\rem{\textcolor{blue}{$\bullet$ #1}}}

    \newcommand{\amatya}[1]{\todo[color=blue!100!black!50]{A: #1}}
    \newcommand{\euiwoong}[1]{\todo[color=green!100!black!50]{E: #1}}
\else
    \newcommand{\adi}[1]{#1}
    \newcommand{\eui}[1]{#1}
    \newcommand{\aay}[1]{#1}
    \newcommand{\adir}[1]{}
    \newcommand{\euir}[1]{}
    \newcommand{\aayr}[1]{}
    \newcommand{\euiwoong}[1]{}
    \newcommand{\amatya}[1]{}
\fi


\newcommand{\sat} {\ensuremath{\mathsf{sat}}\xspace}
\newcommand{\unsat} {\mathsf{unsat}}

%problem definitions
\newcommand{\maxcsps} {\textsc{Max-CSP}s\xspace}
\newcommand{\maxcsp} {\textsc{Max-CSP}\xspace}
\newcommand{\ug} {\textsc{Unique Games}\xspace}
\newcommand{\mincsp}{\textsc{Min-CSP}\xspace}
\newcommand{\minkcsp}{\textsc{Min-$k$-CSP}\xspace}
\newcommand{\minksat}{\textsc{Min-$k$-SAT}\xspace}
\newcommand{\kcsp}{$k$-\textsc{CSP}\xspace}
\newcommand{\kcsps}{$k$-\textsc{CSPs}\xspace}
\newcommand{\klin}{$k$-\textsc{LIN}\xspace}
\newcommand{\kand}{$k$-\textsc{AND}\xspace}
\newcommand{\krcsp}[2]{\textsc{$(#1,#2)$-CSP}\xspace}
\newcommand{\ncsp}[1]{\textsc{$#1$-CSP}\xspace}
\newcommand{\mincsps}{\textsc{Min-CSP}s\xspace}
\newcommand{\minsum}{\textsc{Minsum Clustering}\xspace}
\newcommand{\minuncut}{\textsc{Min-Uncut}\xspace}
\newcommand{\mintwo}{\textsc{Min-2-SAT}\xspace}
\newcommand{\maxtwo}{\textsc{Max-2-SAT}\xspace}
\newcommand{\cc} {\textsc{Correlation Clustering}\xspace}
\newcommand{\lra}{\textsc{Low Rank Approximation}\xspace}
\newcommand{\mvd}{\textsc{Metric Violation Distance}\xspace}
\newcommand{\minug} {\textsc{Min-Unique Games}\xspace}

\newcommand{\maxtwosat}{\ensuremath{\textsc{Max-$2$-SAT}}}
\newcommand{\maxcut}{\ensuremath{\textsc{Max-Cut}}}
\newcommand{\maxbisec}{\ensuremath{\textsc{Max-Bisection}}}
\newcommand{\maxnaethreesat}{\ensuremath{\textsc{Max-NAE-\mbox{-}3-SAT}}}
\newcommand{\rpr}{\ensuremath{\textsc{RPR$^2$}}}

\newcommand{\nae}{\ensuremath{\textsc{NAE-$3$-SAT}}}

\newcommand{\nsat}[1]{\ensuremath{\textsc{$#1$-SAT}}\xspace}

\newcommand{\nand}[1]{\ensuremath{\textsc{$#1$-AND}}\xspace}
\newcommand{\nlin}[1]{\ensuremath{\textsc{$#1$-LIN}}\xspace}
\newcommand{\ksat}{\nsat{k}}
\newcommand{\foursat}{\nsat{4}}
\newcommand{\threesat}{\nsat{3}}
\newcommand{\twosat}{\nsat{2}}

\newcommand{\onlyone}{\ensuremath{\textsc{Only-$1$}}\xspace}
\newcommand{\notone}{\ensuremath{\textsc{Not-$1$}}\xspace}
\newcommand{\threeand}{\ensuremath{\textsc{$3$-AND}}\xspace}
\newcommand{\threelin}{\ensuremath{\nlin{3}}}
\newcommand{\atleasttwo}{\ensuremath{\textsc{At Least-$2$}}\xspace}
\newcommand{\allnone}{\ensuremath{\textsc{All\mbox{-}or\mbox{-}None}}\xspace}
\newcommand{\cnf}{\ensuremath{\textsc{CNF}}\xspace}
\newcommand{\csp}{\ensuremath{\textsc{CSP}}\xspace}


\newcommand{\pac}[1]{\ensuremath{\textsc{$(#1)$\mbox{-}PAC}}\xspace}

\newcommand{\itwosat}[1]{\ensuremath{\textsc{$#1$\mbox{-}Induced\twosat}}\xspace}
\newcommand{\kitwosat}{\itwosat{k}}

\newcommand{\itwocsp}[1]{\ensuremath{\textsc{$#1$\mbox{-}Induced\ncsp{2}}}\xspace}
\newcommand{\kitwocsp}{\itwocsp{k}}




\newcommand{\vareps}{\varepsilon}
\newcommand{\norm}[1]{\ensuremath{\left\lVert#1\right\rVert}}
\newcommand{\lee}{\leqslant}
\newcommand{\gee}{\geqslant}
\newcommand{\ceil}[1]{{\left\lceil{#1}\right\rceil}}
\newcommand{\floor}[1]{{\left\lfloor{#1}\right\rfloor}}
\newcommand{\prob}[1]{\Pr\paren{#1}}
\newcommand{\expect}[1]{\Exp\bracket{#1}}
\newcommand{\var}[1]{\textnormal{Var}\bracket{#1}}
\newcommand{\cov}[1]{\textnormal{Cov}\bracket{#1}}
\newcommand{\eexp}[1]{\exp\paren{#1}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\poly}{\mbox{\rm poly}}
\newcommand{\polylog}{\mbox{\rm  polylog}}
\newcommand{\logstar}[1]{\ensuremath{\log^{*}\!{#1}}}
\newcommand{\logr}[1]{\ensuremath{\log^{(#1)}}}
\newcommand{\APX}{\ensuremath{\mbox{APX}}}
\newcommand{\apx}{\ensuremath{\mbox{apx}}}
\newcommand{\ALG}{\ensuremath{\mbox{\sc alg}}\xspace}
\newcommand{\lp}{\ensuremath{\mathrm{LP}}}
\newcommand{\alg}{\ensuremath{\mathrm{ALG}}}
\newcommand{\opt}{\ensuremath{\mathrm{OPT}}}
\newcommand{\sdp}{\ensuremath{\mathsf{sdp}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\bigO}[1]{\ensuremath{O\Paren{#1}}}
\newcommand{\dist}{\ensuremath{\mathrm{dist}}}

\newcommand{\etal}{{\it et al.\,}}



% Probabilistic notation:  
% \renewcommand{\Pr}{\Prob}
\newcommand{\rv}[1]{\ensuremath{{\mathsf{#1}}}\xspace}
%gaussian, normal
\newcommand{\gaussian}{\normalrv}
%Lebesgue Measure
\newcommand{\vol}{\text{Vol}}
%Transpose
\newcommand{\transpose}{\intercal}
%Inverse
\newcommand{\inverse}{{-1}}
%Operator norm
\newcommand{\opnorm}[1]{\norm{#1}_{\mathsf{op}}}
%Trace
\newcommand{\tr}{\mathsf{Tr}}
\newcommand{\argmax}{\mathrm{argmax}}



% macros for matrices and vectors
\newcommand{\veczero}{\ensuremath{\mathbf{0}}}
\newcommand{\vecdelta}{\ensuremath{\mathbf{\delta}}}
\newcommand{\mA}{\ensuremath{\mathbf{A}}}
\newcommand{\mB}{\ensuremh{\mathbf{B}}}
\newcommand{\mC}{\ensuremath{\mathbf{C}}}
\newcommand{\mD}{\ensuremath{\mathbf{D}}}
\newcommand{\mE}{\ensuremath{\mathbf{E}}}
\newcommand{\mF}{\ensuremath{\mathbf{F}}}
\newcommand{\mG}{\ensuremath{\mathbf{G}}}
\newcommand{\mH}{\ensuremath{\mathbf{H}}}
\newcommand{\mI}{\ensuremath{\mathbf{I}}}
\newcommand{\mJ}{\ensuremath{\mathbf{J}}}
\newcommand{\mK}{\ensuremath{\mathbf{K}}}
\newcommand{\mL}{\ensuremath{\mathbf{L}}}
\newcommand{\mM}{\ensuremath{\mathbf{M}}}
\newcommand{\mN}{\ensuremath{\mathbf{N}}}
\newcommand{\mO}{\ensuremath{\mathbf{O}}}
\newcommand{\mP}{\ensuremath{\mathbf{P}}}
\newcommand{\mQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\mR}{\ensuremath{\mathbf{R}}}
\newcommand{\mS}{\ensuremath{\mathbf{S}}}
\newcommand{\mT}{\ensuremath{\mathbf{T}}}
\newcommand{\mU}{\ensuremath{\mathbf{U}}}
\newcommand{\mV}{\ensuremath{\mathbf{V}}}
\newcommand{\mW}{\ensuremath{\mathbf{W}}}
\newcommand{\mX}{\ensuremath{\mathbf{X}}}
\newcommand{\mY}{\ensuremath{\mathbf{Y}}}
\newcommand{\mZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\mzero}{\ensuremath{\mathbf{0}}}

\newcommand{\veca}{\ensuremath{\mathbf{a}}}
\newcommand{\vecb}{\ensuremath{\mathbf{b}}}
\newcommand{\vecc}{\ensuremath{\mathbf{c}}}
\newcommand{\vecd}{\ensuremath{\mathbf{d}}}
\newcommand{\vece}{\ensuremath{\mathbf{e}}}
\newcommand{\vecf}{\ensuremath{\mathbf{f}}}
\newcommand{\vecg}{\ensuremath{\mathbf{g}}}
\newcommand{\vech}{\ensuremath{\mathbf{h}}}
\newcommand{\vecell}{\ensuremath{\bm{\ell}}}
\newcommand{\veck}{\ensuremath{\mathbf{k}}}
\newcommand{\vecm}{\ensuremath{\mathbf{m}}}
\newcommand{\vecp}{\ensuremath{\mathbf{p}}}
\newcommand{\vecq}{\ensuremath{\mathbf{q}}}
\newcommand{\vecr}{\ensuremath{\mathbf{r}}}
\newcommand{\vecs}{\ensuremath{\mathbf{s}}}
\newcommand{\vect}{\ensuremath{\mathbf{t}}}
\newcommand{\vecu}{\ensuremath{\mathbf{u}}}
\newcommand{\vecv}{\ensuremath{\mathbf{v}}}
\newcommand{\vecw}{\ensuremath{\mathbf{w}}}
\newcommand{\vecx}{\ensuremath{\mathbf{x}}}
\newcommand{\vecy}{\ensuremath{\mathbf{y}}}
\newcommand{\vecz}{\ensuremath{\mathbf{z}}}

\newcommand{\vecA}{\ensuremath{\mathbf{A}}}
\newcommand{\vecB}{\ensuremath{\mathbf{B}}}
\newcommand{\vecC}{\ensuremath{\mathbf{C}}}
\newcommand{\vecD}{\ensuremath{\mathbf{D}}}
\newcommand{\vecE}{\ensuremath{\mathbf{E}}}
\newcommand{\vecF}{\ensuremath{\mathbf{F}}}
\newcommand{\vecG}{\ensuremath{\mathbf{G}}}
\newcommand{\vecH}{\ensuremath{\mathbf{H}}}
\newcommand{\vecI}{\ensuremath{\mathbf{I}}}
\newcommand{\vecJ}{\ensuremath{\mathbf{J}}}
\newcommand{\vecK}{\ensuremath{\mathbf{K}}}
\newcommand{\vecL}{\ensuremath{\mathbf{L}}}
\newcommand{\vecM}{\ensuremath{\mathbf{M}}}
\newcommand{\vecN}{\ensuremath{\mathbf{N}}}
\newcommand{\vecO}{\ensuremath{\mathbf{O}}}
\newcommand{\vecP}{\ensuremath{\mathbf{P}}}
\newcommand{\vecQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\vecR}{\ensuremath{\mathbf{R}}}
\newcommand{\vecS}{\ensuremath{\mathbf{S}}}
\newcommand{\vecT}{\ensuremath{\mathbf{T}}}
\newcommand{\vecU}{\ensuremath{\mathbf{U}}}
\newcommand{\vecV}{\ensuremath{\mathbf{V}}}
\newcommand{\vecW}{\ensuremath{\mathbf{W}}}
\newcommand{\vecX}{\ensuremath{\mathbf{X}}}
\newcommand{\vecY}{\ensuremath{\mathbf{Y}}}
\newcommand{\vecZ}{\ensuremath{\mathbf{Z}}}


\newcommand{\A}{\ensuremath{\mathbb{A}}}
\newcommand{\rA}{\ensuremath{\mathrm{A}}}
\newcommand{\bA}{\ensuremath{\mathbf{A}}}
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathbb{B}}}
\newcommand{\rB}{\ensuremath{\mathrm{B}}}
\newcommand{\bB}{\ensuremath{\mathbf{B}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\rC}{\ensuremath{\mathrm{C}}}
\newcommand{\bC}{\ensuremath{\mathbf{C}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathbb{D}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\rD}{\ensuremath{\mathrm{D}}}
\newcommand{\bD}{\ensuremath{\mathbf{D}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\rE}{\ensuremath{\mathrm{E}}}
\newcommand{\bE}{\ensuremath{\mathbf{E}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\rF}{\ensuremath{\mathrm{F}}}
\newcommand{\bF}{\ensuremath{\mathbf{F}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\G}{\ensuremath{\mathbb{G}}}
\newcommand{\rG}{\ensuremath{\mathrm{G}}}
\newcommand{\bG}{\ensuremath{\mathbf{G}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\rH}{\ensuremath{\mathrm{H}}}
\newcommand{\bH}{\ensuremath{\mathbf{H}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}
\newcommand{\rI}{\ensuremath{\mathrm{I}}}
\newcommand{\bI}{\ensuremath{\mathbf{I}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\J}{\ensuremath{\mathbb{J}}}
\newcommand{\rJ}{\ensuremath{\mathrm{J}}}
\newcommand{\bJ}{\ensuremath{\mathbf{J}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\K}{\ensuremath{\mathbb{K}}}
\newcommand{\rK}{\ensuremath{\mathrm{K}}}
\newcommand{\bK}{\ensuremath{\mathbf{K}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
% \newcommand{\L}{\ensuremath{\mathbb{L}}}
\newcommand{\rL}{\ensuremath{\mathrm{L}}}
\newcommand{\bL}{\ensuremath{\mathbf{L}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\M}{\ensuremath{\mathbb{M}}}
\newcommand{\rM}{\ensuremath{\mathrm{M}}}
\newcommand{\bM}{\ensuremath{\mathbf{M}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\rN}{\ensuremath{\mathrm{N}}}
\newcommand{\bN}{\ensuremath{\mathbf{N}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
% \newcommand{\O}{\ensuremath{\mathbb{O}}}
\newcommand{\rO}{\ensuremath{\mathrm{O}}}
\newcommand{\bO}{\ensuremath{\mathbf{O}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
% \newcommand{\P}{\ensuremath{\mathbb{P}}}
\newcommand{\rP}{\ensuremath{\mathrm{P}}}
\newcommand{\bP}{\ensuremath{\mathbf{P}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\rQ}{\ensuremath{\mathrm{Q}}}
\newcommand{\bQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\cQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\rR}{\ensuremath{\mathrm{R}}}
\newcommand{\bR}{\ensuremath{\mathbf{R}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
% \newcommand{\S}{\ensuremath{\mathbb{S}}}
\newcommand{\rS}{\ensuremath{\mathrm{S}}}
\newcommand{\bS}{\ensuremath{\mathbf{S}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\rT}{\ensuremath{\mathrm{T}}}
\newcommand{\bT}{\ensuremath{\mathbf{T}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}
\newcommand{\rU}{\ensuremath{\mathrm{U}}}
\newcommand{\bU}{\ensuremath{\mathbf{U}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\V}{\ensuremath{\mathbb{V}}}
\newcommand{\rV}{\ensuremath{\mathrm{V}}}
\newcommand{\bV}{\ensuremath{\mathbf{V}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\W}{\ensuremath{\mathbb{W}}}
\newcommand{\rW}{\ensuremath{\mathrm{W}}}
\newcommand{\bW}{\ensuremath{\mathbf{W}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\rX}{\ensuremath{\mathrm{X}}}
\newcommand{\bX}{\ensuremath{\mathbf{X}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\rY}{\ensuremath{\mathrm{Y}}}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\rZ}{\ensuremath{\mathrm{Z}}}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}

\newcommand{\bone}{\overline{1}}

==> Inputs/kcsp-old.tex <==
\iffalse 
\section{\texorpdfstring{$\ksat$}{kSAT} Decision Version}
\label{sec:ksat}

    We first illustrate the idea using the example of $\foursat$. And, then in \Cref{sec:ksat}, we give the quasi-polynomial time decision algorithm for general $\ksat$.
    \subsection{\texorpdfstring{$\foursat$}{4SAT} Algorithm}
    
        Given an instance $(V, \calC)$ where each $4$-tuple of variables $(u,v,w,x)$ corresponds to exactly one clause $(\ell_u, \ell_v, \ell_w, \ell_x) \in \calC$, let $\alpha : V \to \{ 0, 1 \}$ be an arbitrary satisfying assignment. Our algorithm proceeds in rounds, and each round makes $\poly(n)$ guesses about $\alpha$. Ideally, one of the guesses will allow us to correctly identify the $\alpha$ values for $\Omega(n)$ variables so that the recursion will yield a quasi-polynomial time algorithm.
        
        
        In the case where all $\poly(n)$ guesses fail, we can produce a complete \threesat instance which is guaranteed to satisfy by $\alpha$. Thus, it suffices to enumerate all the \threesat solutions for the produced instance and see whether they are good for the original \foursat. 


        Given the enumeration algorithm for \threesat (\Cref{alg:3satassgn}), we now present our main subroutine for \foursat. 
        \paragraph{Overview.}
        Let $\alpha : V \to \{ 0, 1 \}$ be one of the satisfying assignments we are interested in. 
        For a $3$-tuple of variables $v_i,v_j, v_k\in V$, assume that the optimal assignment $\alpha(v_i) = \alpha(v_j) = \alpha(v_k)= 1$. Then, every clause --- out of the total $n-3$ clauses containing the $3$-tuple --- of the form $(\neg v_i, \neg v_j,\neg v_k \ell)$ must fix the fourth literal to true. We define this formally as follows:
        

        
        \begin{definition}[Fixed Variables]\label{def:4satmaj}
            Given every set of three variables $(v_{i_1},v_{i_2}, v_{i_3})\in \binom{V}{3}$ and every pair of possible values of $v_{i_1},v_{i_2}, v_{i_3}$, say $(a_1, a_2, a_3)\in\{0,1\}^3$. We define $n_{i_1, i_2, i_3,a_1, a_2, a_3}$ as the total number of clauses of the form $(s_{i_1}v_{i_1},s_{i_2}v_{i_2}, s_{i_3}v_{i_3}, \ell)\in \cC$, for literals $\ell$ for all the variables $v\in V\setminus \{v_{i_1},v_{i_2}, v_{i_3}\}$, where the sign $s_{i_j}\in[\perp, \neg]$ is positive ($\perp$) if $a_{i_j}=0$, and negative ($\neg$) otherwise, for all $j\in[3]$. Moreover, define the corresponding set of fixed literals $\ell$ as $N_{i_1, i_2, i_3,a_1, a_2, a_3}$.
        \end{definition}
        

        Call $(v_i, v_j,v_k)$ a \emph{good $3$-tuple  with respect to $\alpha$} if the value $n_{i,j,k,\alpha(v_i),\alpha(v_j), \alpha(v_k)}\geq \eps_4 n$. So guessing the values $\alpha(v_i)$, $\alpha(v_j)$ and $\alpha(v_k)$ correctly (w.r.t. $\alpha$), fixes at least $\eps_4 n$ variables. 
        If we can iterate this process for $\frac{\log n}{\eps_4}$ iterations, we will fix all variables and find $\alpha$. 
    
    
        Now, consider the case where for every $3$-tuple $(v_i, v_j,v_k)$, we have $n_{i,j,k,\alpha(i), \alpha(j), \alpha(k)} < \eps_4 n$. Thus, $(a', b',c') := \arg \max_{(a,b,c)} n_{i,j,k,a,b,c}$ can not be the same as $(\alpha(i), \alpha(j), \alpha(k))$ (for any $\eps_4 \leq \frac{1}{32})$. We add a \threesat constraint $(v_i, v_j, v_k)\neq (a',b', c')$, which is surely satisfied by $\alpha$. Doing the same for all pairs, we get a complete \threesat instance. From \Cref{lem:satnumberassgn}, we know that the number of satisfiable assignments for a complete \threesat instance on $n$ variables can be at most $O(n^2)$, and these can be computed in time $n^{O(\log n)}$ (\Cref{thm:3satassgn}). Thus, we can enumerate all the satisfying assignments to the created \threesat instance, and $\alpha$ will be one of them. 

        
        
        \paragraph{Algorithm.} The \Cref{alg:4satassgn} takes in input as the variables $V$, the complete instance clauses $\cC$, and an partial assignment to all the literals $\alpha:V\mapsto\{0,1,\frac12\}$ where for any undecided variable $v$, $\alpha(v) = \frac12$. Initially, the assignment $\alpha$ is completely undecided, i.e., $\alpha(v)=\frac12$ for all $v\in V$. It outputs $\cA$, which will eventually be all satisfying assignments to $(V, \cC)$. 


        The algorithm first computes the set of unfixed variables $V_U = \{v\in V\ |\ \alpha(v) = \frac12\}$. In Step \ref{alg4satassgnstep:lessvars}, if there are only $O(\log n)$ unfixed variables, we enumerate all assignments and check whether they give a satisfying assignment. This takes time $2^{|V_U|} \cdot \poly(n) = \poly(n)$.
        

        The algorithm branches by either guessing one of the good $3$-tuples (Step \ref{alg4satassgnstep:guess}) and their assignment, or assuming that there are no good $3$-tuples, forms a complete \threesat instance (Step \ref{alg4satassgnstep:2sat}). 
    
    
        In Step \ref{alg4satassgnstep:guess}, we guess a $3$-tuple $(v_i, v_j, v_k)$ by branching over all $3$-tuples of unfixed variables and guess their optimal assignment $(a,b,c)$. If the guessed $3$-tuple is a good $3$-tuple with respect to some satisfying assignment $\alpha$, i.e., if $n_{i,j,k, \alpha(v_i),\alpha(v_j), \alpha(v_k)}\geq |V_U|/16$, then we can correctly fix at least $\eps_4 |V_U|$ variables $N_{i,j,k, \alpha(v_i),\alpha(v_j), \alpha(v_k)}$ and solve the problem recursively. Thus we only need to recurse to depth at most $\frac{\log n}{\eps_4}$ before fixing all the variables optimally. This is ensured by Step \ref{alg4satassgnstep:depth}. 
    
    
        In Step \ref{alg4satassgnstep:2sat}, we branch by assuming that there is no good $3$-tuple with respect to $\alpha$ among the unfixed variables. Under this assumption, we know that $n_{i,j,k, \alpha(v_i),\alpha(v_j), \alpha(v_k)}< \eps_4 V_U|$. Since, all the eight quantities $n_{i,j,k, a,b, c}$ over all $a,b, c\in\{0,1\}$ sum up to $|V_U|-3$, defining $(a', b', c') := \mathrm{argmax}_{(a,b, c)\in\{0,1\}}n_{i,j, k,a,b, c}$ (while arbitrarily breaking ties) ensures that $(\alpha(v_i), \alpha(v_j), \alpha(v_k)) \neq (a', b', c')$. %, which allows us to put a \twosat constraint that the $3$-tuple $(v_i, v_j)$ can notbe assigned $(a', b')$. 
        So, we add the \threesat constraints $(v_i, v_j, v_k)\neq (a', b', c')$ for all $v_i, v_j, v_k\in V$. This gives us a complete \threesat instance $\cC_3$ over the unfixed variables that is guaranteed to be satisfied by $\alpha$. In Steps \ref{alg4satassgnstep:find2sat} and \ref{alg4satassgnstep:check2sat}, we compute and check whether any of the satisfiable assignments of the \threesat instance $\cC_3$ satisfy the \foursat instance $\cC$ or not. We add every such satisfying assignment to the set $\cA$.

        
        \begin{algorithm}
            \caption{ALG-$\foursat$-decision$_{\cA}(V,\cC,\alpha, d)$}
            \label{alg:4satassgn}
            \begin{algorithmic}[1]
                \Require $V, \cC, \alpha:V\mapsto \{\frac12, 1, 0\}, d$
                \State $\mathrm{ret}\gets 0$ \Comment{Value to return, $0$ if unsatisfied, and $1$ otherwise}
                \IIf{$d>10 \frac{1}{\eps_4}\log |V|$} \label{alg4satassgnstep:depth}
                    \Return %$\mathrm{ret}$ \Comment{If depth exceeds $O(\log n)$, return $0$}
                \EndIIf
                \State $V_U \gets \{v\in V\ |\ \alpha(v)\neq\frac12\}$ and $V_F \gets V\setminus V_U$\label{alg4satassgnstep:unfix1}
                \Comment{unfixed and fixed variables}
                % \State $\cC_U \gets \{C\ | C\cap \{V_F,\neg V_F\} = \emptyset, \forall C\in \cC\}$ \Comment{complete instance induced on unfixed variables}\label{alg4satassgnstep:unfix2}
                \If{$|V_U|\leq 100 \log n$} \label{alg4satassgnstep:lessvars}
                    % \State Guess optimal assignment $\alpha(V_U)$ of all variables in $V_U$.
                    % \If{check-assignment($V, \cC, \alpha)=1$}
                    %     \State $\mathrm{ret}\gets 1$.
                    %     \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    % \EndIf
                    \State For each assignment to $\alpha : V_U \to \{ 0, 1\}$, if the entire $\alpha$ satisfies $\calC$, add $\alpha$ to $\cA$. 
                \EndIf
                \For{all $(v_i, v_j, v_k)\in \binom{V_U}{3}$}\label{alg4satassgnstep:guess}\Comment{Guess a $3$-tuple}
                    \For{all $(a,b,c)\in \{0,1\}^3$}\Comment{Guess the optimal assignment}
                        \If{$n_{i, j, k, a,b,c} \geq \eps_4 |V_U|$}
                            \State Let $\alpha'$ be the extension of $\alpha$ where $\alpha'(v_i) \leftarrow a, \alpha'(v_j) \leftarrow b, \alpha'(v_k)\gets c$ and 
                            \State $\quad \quad \alpha'(v) \leftarrow a$ for every $v \in N_{i,j,k, a, b,c}$. 
                            % \State Set $\alpha(v_{i_j}) \gets a_j$ for all $j\in[3]$.
                            % \State Set $\alpha(v)$ for all $v$ with literal $\ell\in N_{i_1, i_2, i_3,a_1, a_2, a_3}$ to $1$. 
                            \State ALG-$\foursat$-decision$_{\cA}(V, \cC, \alpha', d+1)$.
                            % \State Set $\alpha(v_{i_j}), \alpha(v) \gets \frac12$ for all $j\in[3]$. \Comment{After the recursive call, reset}
                        \EndIf
                    \EndFor
                \EndFor
                \State $\cC_3\gets \emptyset$ \Comment{Set of \threesat constraints} 
                \For{all $(v_i, v_j, v_k)\in \binom{V_U}{3}$}\label{alg4satassgnstep:2sat}\Comment{Otherwise add \threesat constraints}
                    \State $(a',b',c') \gets \arg\max_{(a,b,c))\in \{0,1\}^3} n_{i,j,k, a, b,c}$ \Comment{Find the maximum value}
                    \State Add \threesat constraint $\cC_3\gets \cC_3\cup ((v_i, v_j, v_k)\neq(a',b',c'))$
                \EndFor
                \State Compute $\cA(V_U, \cC_3)$. \label{alg4satassgnstep:find2sat}\Comment{Compute all the satisfiable assignments of the complete \threesat instance}
                \For{$\alpha' \in \cA(V_U,\cC_3)$}\label{alg4satassgnstep:check2sat}\Comment{Enumerate over all satisfiable complete \threesat assignments}
                    \State $\alpha(V_U)\gets \alpha'(V_U)$. \Comment{Set the partial $\foursat$ assignment based on $\threesat$ assignment}
                    \IIf{check-assignment($V,\cC,\alpha) =1$}
                        % \State $\mathrm{ret}\gets 1$.
                        \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    \EndIIf \Comment{Return $1$ if some branch finds a satisfiable assignment}
                \EndFor
                % \State Remove-duplicates$(\cA)$.
                % \State \Return $\mathrm{ret}$. \Comment{Return $0$ if none of the branches find a satisfiable assignment}
            \end{algorithmic}
        \end{algorithm}
            
        \paragraph{Correctness.} For the correctness of the algorithm, we need to prove that the algorithm outputs the set of all the satisfying assignments to the instance.
        We now prove that the set of satisfying assignments $\cA$ of the algorithm contains all the satisfying assignments to the instance.
    
        \begin{lemma}\label{lem:4satallassgn}
            Every satisfying assignment $\alpha^*$ belongs to $\cA$.
        \end{lemma}
        \begin{proof}
            Consider any satisfying assignment $\alpha^*$. We prove that in each recursive call, 
            (Case 1) if there exists a good $3$-tuple $(v_i, v_j, v_k)$ with respect to $\alpha^*$, we will correctly fix at least $ \eps_4|V_U|$ values of $\alpha^*$ in one of the branches, and 
            (Case 2) if there is no good $3$-tuple, we create a complete \threesat instance satisfied by $\alpha^*$. 
            If this is true, then in at most $ \frac{\log n}{\eps_4}$ recursive depth, we would end up guessing $\alpha^*$ in at least one leaf and return $1$ and store $\alpha^*$ in $\cA$.
            
            \paragraph{Case 1: Branching over good-$3$-tuples:} Suppose that for some $3$-tuple $(v_i,v_j, v_k)$ is good $3$-tuple w.r.t $\alpha^*$; i.e., $n_{v_i, v_j, v_k, \alpha^*(v_i,v_j, v_k)} \geq |V_U|/16$. Then the algorithm would branch over this choice of $v_i,v_j, v_k, \alpha^*(v_i,v_j, v_k)$ as it branches over all the possible choices of good $3$-tuples. Then, the algorithm sets $\alpha^*(v_i,v_j, v_k)$ as well as $\alpha^*(N_{v_i,v_j, v_k \alpha^*(v_i,v_j, v_k)})$ correctly (follows from the \Cref{def:4satmaj} of fixed variables). 
            
            
            \paragraph{Case 2: Branching over complete \threesat:} If in a recursive call of the algorithm, for no $3$-tuple $(v_i,v_j, v_k)\in \binom{V_U}{3}$, we have that $n_{v_i,v_j, v_k,\alpha^*(v_i,v_j, v_k)} \geq \eps_4|V_U|$, then consider the branch where the algorithm forms a complete \threesat on the unfixed variables $V_U$ in Step \ref{alg4satassgnstep:2sat}. 
            (Note that the $3$-tuple $v_i, v_j, v_k$ can still be a good $3$-tuple w.r.t. some other optimal assignment $\alpha^{**}$.)
            We claim that the complete \threesat instance is satisfiable by assignment $\alpha^*(V_U)$, which is the restriction of $\alpha^*$ to $V_U$. 

    
            If this were true, then we would be done as we branch over all the possible \threesat assignments to $V_U$, and $\alpha^*(V_U)$ must be one of them. 
            
            Fix any $3$-tuple $(v_i, v_j, v_k) \in \binom{V_U}{3}$. 
            We know that $n_{v_i,v_j, v_k, \alpha^*(v_i,v_j, v_k)}< \eps_4|V_U|$. 
            Since, all the $8$ quantities $n_{v_i,v_j,\alpha(v_i,v_j)}$, over all $\alpha(v_i,v_j, v_k)\in\{0,1\}^{3}$, sum up to $|V_U|-3$, the $\max_{\alpha(v_i,v_j, v_k)\in\{0,1\}^{3}}n_{v_i,v_j, v_k,\alpha(v_i,v_j, v_k)}$ must be at least $\frac{|V_U|-3}{8}\aay{\geq\frac{|V_U|}{16}}$ (as $|V_U|>\Omega(\log n)$, and $n$ is large enough) by averaging argument. This maximum value does not correspond to the $n_{v_i,v_j, v_k, \alpha^*(v_i,v_j, v_k)}$ value for any $\eps_4 \leq \frac{1}{32}$. Since this $3$-tuple $\alpha(v_i, v_j, v_k)$ that achieves the maximum is exactly what our added \threesat constraint rules out, $\alpha^*(v_i, v_j, v_k)$ will satisfy this constraint. 
        \end{proof} 
    
       
        

    \paragraph{Analysis.} The algorithm either branches over all the $8\cdot \binom{|V_U|}{3}$ number of guesses of $3$-tuples and their assignments, or formulates the complete \threesat instance $\cC_3$ on $V_U$, and checks whether any \threesat assignment satisfies the \foursat instance $\cC$ or not. Since, the former fixes at least $\eps_4 |V_U|$ variables, the depth of the branching tree would be at most $\frac{\log n}{\eps_4}$ before we can correctly arrive at a conclusion. For the latter, we know that all the assignments to $V_U$ satisfying the \threesat instance $\cC_3$ can be found in $n^{O(\log n)}$ time (this bounds the number of assignments as well).
    Since there are at most $(8n^{3})^{\frac{\log n}{\eps_4}}$ recursive calls and each call takes $n^{O(\log n)}$ time, the total runtime of the algorithm is $n^{O(\log n)} \cdot (8n^{3})^{\frac{\log n}{\eps_4}} = n^{O(\log n)}$, for $\eps_4=\frac{1}{32}$ which yields the following theorem. 
    
    
        \begin{theorem}\label{thm:4satassgn}
            There is a $n^{O(\log n)}$ time algorithm to decide whether a complete instance of $\foursat$ on $n$ variables is satisfiable or not. Moreover, this algorithm also returns all the $O(n^3)$ satisfying assignments.
        \end{theorem}
        


    \subsection{\texorpdfstring{$\ksat$}{kSAT} Algorithm}%\label{sec:ksat}
        
        The goal is to recursively construct and output the set of all the optimal assignments. Note that by optimal assignment, we mean the assignment that satisfies the entire instance. If all optimal assignments is non-empty, we recursively construct and output the entire set. If the solution is an empty set then, we conclude that the instance is unsatisfiable.

        \paragraph{Overview.} The idea is similar to the \foursat problem. If in an optimal assignment, there is a clause that has all the literals corresponding to the $k-1$ variables set to false, then we have to fix the $k$'th literal to true to satisfy the clause. The number of clauses any $k-1$ variables appear in as literals is at least $n-k+1$. We call a set of $k-1$ variables a \emph{Good $(k-1)$-tuple}, if for some optimal assignment the number of such clauses (or equivalently the number of variables fixed by the assignment) is at least $\eps n$. Thus, the algorithm guesses the good $k$-tuple out of $\binom{n}{k}$ possibilities, guesses the optimal assignment to the tuple, fixes the $\Omega(n)$ variables, and, proceeds recursively.



        We will see that in the other case when there are no such good tuples, the algorithm can add complete $\nsat{(k-1)}$ constraints on all the unfixed variables. Using induction, we can use the algorithm for $\nsat{(k-1)}$, to compute all the $O(n^{k-2})$ $\nsat{(k-1)}$ assignments in time $n^{O(\log n)}$ and check whether any of these satisfies the $\ksat$ instance or not. 
        

        Given every set of $k-1$ variables $\vecv\in V^{k-1}$ and every tuple of possible values of $\vecv$, say $\alpha(\vecv)\in\{0,1\}^{k-1}$. For literals $\ell'$ for all the variables $v\in V\setminus \vecv$, we call a clause of the form $(\vecell,\ell')\in \cC$ a \emph{fixed} clause, where $\vecell$ correspond to some literals of $\vecv$, if all the $k-1$ literals $\vecell$ are assigned $0$, i.e., the assignment of the last undecided literal $\ell'$ is fixed.
        \begin{definition}[Fixed Variables]\label{def:ksatmaj}
            Define $n_{\vecv, \alpha(\vecv)}$ as the total number of fixed clauses for the $(k-1)$-tuple $\vecv$ and their assignment $\alpha(\vecv)$. Moreover, define the corresponding set of fixed literals $\ell'$ that are fixed as $N_{\vecv, \alpha(\vecv)}$.
        \end{definition}

        \paragraph{Algorithm.} The \Cref{alg:ksatassgn} takes in input as the variables $V$, the complete instance clauses $\cC$, and an partial assignment to all the literals $\alpha:V\mapsto[0,1,\frac12]$. For any variable $v$, if the assignment is undecided $\alpha(v) = \frac12$. Initially, the assignment $\alpha$ is completely undecided, i.e., $\alpha(v)=\frac12$ for all $v\in V$.

    
        In Step \ref{algksatassgnstep:lessvars}, we first directly guess the optimal value of the unfixed variables if there are only $O(\log n)$ many of them. This takes time $2^{|V_U|} = \poly(n)$. Then, in another $\poly(n)$, we check whether the whole assignment satisfies all the clauses of the $\ksat$ instance. If yes, we add the assignment $\alpha$ to the set of all satisfying assignments $\cA$.
    
        The algorithm branches by either guessing one of the good $(k-1)$-tuples (Step \ref{algksatassgnstep:guess}) and their assignment, or assuming that there are no good tuples and forms a complete $\nsat{(k-1)}$ instance (Step \ref{algksatassgnstep:2sat}). If any of the branches returns that there is a satisfying assignment, we conclude that the instance is satisfiable. Otherwise, if none of the branches return that there is a satisfiable assignment, then we conclude that the instance is unsatisfiable. 
        
        
        In Step \ref{algksatassgnstep:guess}, we guess a $(k-1)$-tuple $\vecv$ by branching over all tuples of unfixed variables and guess their optimal assignment $\alpha^*(\vecv)$. If the guessed tuple (for the guessed optimal value) is a good tuple, i.e., if $n_{\vecv, \alpha^*(\vecv)}\geq \eps|V_U|$, then we can correctly fix at least $\eps|V_U|$ variables $N_{\vecv, \alpha^*(\vecv)}$ and solve the problem recursively. We only need to recurse to depth at most $O(\frac{1}{\eps}\log n)$ before fixing all the variables optimally. This is ensured by Step \ref{algksatassgnstep:depth}. 
        
        
        In Step \ref{algksatassgnstep:2sat}, we branch by assuming that there is no good $(k-1)$-tuple among the unfixed variables. Under this assumption, we know that $n_{\vecv,\alpha^*(\vecv)}< \eps|V_U|$ for all optimal assignments $\alpha^*$. Since, all the $2^{k-1}$ quantities $n_{\vecv,\alpha(\vecv)}$ over all $\alpha(\vecv)\in\{0,1\}^{k-1}$ sum up to $|V_U|-k+1$, the $\max_{\alpha(\vecv)\in\{0,1\}^{k-1}}n_{\vecv,\alpha(\vecv)}$ must be at least $\frac{1}{2^{k}}|V_U|$ by averaging argument. Thus, for any $\eps <\frac{1}{2^{k}}$, this maximum value can not correspond to the $n_{\vecv, \alpha^*(\vecv)}$ value. This gives us an (\nsat{(k-1)}) constraint that the $(k-1)$-tuple $\vecv$ can not be assigned $(\alpha'(\vecv))$ that maximizes $\max_{\alpha(\vecv)\in\{0,1\}^{k-1}}n_{\vecv,\alpha(\vecv)}$. So, we add the \nsat{(k-1)} constraints $\vecv\neq \alpha'(\vecv)$ for all $\vecv\in V_U^{k-1}$. This gives us a complete $\nsat{(k-1)}$ instance $\cC_{k-1}$ over the unfixed variables that is satisfiable if and only if the original instance is satisfiable (under the assumption). In Steps \ref{algksatassgnstep:find2sat} and \ref{algksatassgnstep:check2sat}, we compute and check whether all the satisfiable assignments of the $\nsat{(k-1)}$ instance $\cC_{k-1}$ satisfy the $\nsat{(k-1)}$ instance $\cC$ or not. We add every such satisfying assignment to the set $\cA$.


         
        \begin{algorithm}
            \caption{ALG-$\ksat$-decision$_{\cA}(V,\cC,\alpha, d)$}
            \label{alg:ksatassgn}
            \begin{algorithmic}[1]
                \Require $V, \cC, \alpha:V\mapsto \{\frac12, 1, 0\}, d$
                % \State $\mathrm{ret}\gets 0$ \Comment{Value to return, $0$ if unsatisfied, and $1$ otherwise}
                \If{$d>10 \frac{1}{\eps}\log |V|$} \label{algksatassgnstep:depth}
                    \Return $\mathrm{ret}$ \Comment{If depth exceeds $O(\log n)$, return $0$}
                \EndIf
                \State $V_U \gets \{v\ |\ \alpha(v)\neq\frac12, \forall v\in V\}$ and $V_F \gets V\setminus V_U$\label{algksatassgnstep:unfix1}
                \Comment{unfixed and fixed variables}
                % \State $\cC_U \gets \{c\ | C\cap \{V_F,\neg V_F\} = \emptyset, \forall C\in \cC\}$ \Comment{complete instance induced on unfixed variables}\label{algksatassgnstep:unfix2}
                \If{$|V_U|\leq 100 \log n$} \label{algksatassgnstep:lessvars}
                    % \State Guess optimal assignment $\alpha(V_U)$ of all variables in $V_U$.
                    % \If{check-assignment($V, \cC, \alpha)=1$}
                    %     \State $\mathrm{ret}\gets 1$.
                    %     \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    % \EndIf
                    \State For each assignment to $\alpha : V_U \to \{ 0, 1\}$, if the entire $\alpha$ satisfies $\calC$, add $\alpha$ to $\cA$. 
                \EndIf
                \For{all $\vecv\in V_U^{k-1} $}\label{algksatassgnstep:guess}\Comment{Guess a $(k-1)$-tuple}
                    \For{all $\veca\in \{0,1\}^{k-1}$}\Comment{Guess the optimal assignment}
                        \If{$n_{\vecv,\veca} \geq \eps|V_U|$}
                            \State Set $\alpha(\vecv) \gets \veca$.
                            \State Set $\alpha(v)$ accordingly if it has a literal $\ell\in N_{\vecv, \veca}$ to $1$. 
                            \State $\mathrm{ret}\gets \mathrm{ret}\vee$ALG-$\foursat$-decision$_{\cA}(V, \cC, \alpha, d+1)$.
                            \State Set $\alpha(\vecv),\alpha(v) \gets \frac12$, . \Comment{After the recursive call, reset}
                        \EndIf
                    \EndFor
                \EndFor
                \State $\cC_{k-1}\gets \emptyset$ \Comment{Set of \nsat{(k-1)} constraints} 
                \For{all $\vecv\in V_U^{k-1} $}\label{algksatassgnstep:2sat}\Comment{Otherwise add \nsat{(k-1)} constraints}
                    \State $\veca' \gets \arg\max_{\veca\in \{0,1\}^{k-1} }n_{\vecv, \veca}$ \Comment{Find the maximum value}
                    \State Add \nsat{(k-1)} constraint $\cC_{k-1}\gets \cC_{k-1}\cup ((\vecv)\neq(\veca'))$
                \EndFor
                \State Compute $\cA(V_U, \cC_{k-1})$. \label{algksatassgnstep:find2sat}\Comment{Compute all the satisfiable assignments of the complete \nsat{(k-1)} instance}
                \For{$\alpha' \in \cA(V_U,\cC_{k-1})$}\label{algksatassgnstep:check2sat}\Comment{Enumerate over all satisfiable complete \nsat{(k-1)} assignments}
                    \State $\alpha(V_U)\gets \alpha'(V_U)$. \Comment{Set the partial $\ksat$ assignment based on \nsat{(k-1)} assignment}
                    \If{check-assignment($V,\cC,\alpha) =1$}
                        \State $\mathrm{ret}\gets 1$.
                        \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    \EndIf \Comment{Return $1$ if some branch finds a satisfiable assignment}
                \EndFor
                \State Remove-duplicates$(\cA)$.
                \State \Return $\mathrm{ret}$. \Comment{Return $0$ if none of the branches find a satisfiable assignment}
            \end{algorithmic}
        \end{algorithm}



        \paragraph{Correctness.} At each step the algorithm branches into exactly $2^{k-1}\binom{|V_U|}{k}+1 \leq O(n^{k-1})$ branches. The former term comes from all pairs of unfixed variables, and the latter comes from the last $\nsat{(k-1)}$ branch. It is clear that if (and only if) there exists an (optimal) satisfying assignment to the instance, then the algorithm would return $1$. This is sufficient to check the satisfiability of the $\ksat$ instance and get the following:

        \begin{lemma}\label{lem:ksatsat}
            Every assignment $\cA$ is a satisfying assignment.
        \end{lemma}
         
        We now prove that the set of satisfying assignments $\cA$ of the algorithm contains all the satisfying assignments to the instance.
    
        \begin{lemma}\label{lem:ksatallassgn}
            Every satisfying assignment $\alpha$ belongs to $\cA$.
        \end{lemma}
        \begin{proof}
            The proof is similar to that of $\foursat$ (\Cref{lem:4satallassgn}). 
            Consider any satisfying assignment $\alpha$. If $\alpha$ does not have any good $(k-1)$-tuples $\vecv\in V_U$, then we guess all the possible assignments by enumerating the $\nsat{(k-1)}$ constraints (given by the assignment itself). As we have proved already, the complete \nsat{(k-1)} instance has a satisfying assignment if and only if $\alpha$ is an optimal assignment to the instance. Thus, we guess $\alpha(V_U)$ correctly in this case. Else if $\alpha$ contains some good $(k-1)$-tuples, then the algorithm would definitely branch over all these $(k-1)$-tuples recursively, and guess the correct assignment of these good $(k-1)$-tuples w.r.t $\alpha$. The number of such recursive calls is at most $\frac{2}{\eps}\log n$ as we fix $\eps$ fraction of variables each time. Thus, the algorithm would correctly return $1$ and store the exact assignment $\alpha$ in $\cA$ at the end.
        \end{proof} 
    
    
        \paragraph{Analysis.} The algorithm either branches over all the $|V_U|^{k-1}$ number of guesses of pairs, or formulates the complete $\nsat{(k-1)}$ instance $\cC_{k-1}$ on $V_U$, and checks whether any $\nsat{(k-1)}$ assignment satisfies the $\nsat{(k-1)}$ instance $\cC$ or not. Since, the former fixes at least $\eps|V_U|$ variables, the depth of the branching tree would be at most $\frac{1}{\eps}\log n$ before we can correctly arrive at a conclusion. For the latter, we use induction to establish that all the assignments to $V_U$ satisfying the $\nsat{(k-1)}$ instance $\cC_{k-1}$ can be found in $n^{O(\log n)}$ time (this bounds the number of assignments as well). This also gives us that $|\cA|$ before we remove duplicates can be at most the number of leaves in the recursion tree, i.e., $n^{O(\log n)}$. From \Cref{lem:2satassgn}, we know that the total number of satisfiable assignments (i.e., the total size of $\cA$ after removing duplicates) is at most $O(n^{k-1})$.
        
        
        This would give us the following:
        
        
        \begin{theorem}\label{thm:ksatassgn}
            There is a $n^{O(\log n)}$ time algorithm to decide whether a complete instance of $\ksat$ on $n$ variables is satisfiable or not. Moreover, this algorithm also returns all the $O(n^{k-1})$ satisfying assignments.
        \end{theorem}
\fi


%%%%%%%% kcsp

\section{$k$-CSP}
\label{sec:kcsp}
In this section, we present a quasi-polynomial algorithm for complete $k$-CSP, proving Theorem~\ref{thm:kcsp}; again, in addition to deciding the satisfiability of the instance, our algorithm enumerates all the satisfying assignments. 
    Given an instance $(V, \calC)$ where each $k$-tuple of variables $\vecv \in \binom{V}{k}$
    \euiwoong{$\binom{V}{k}$ is the collection of $k$-sets. Given $C$ is a technically a set as well, it makes sense to change $\vecv$ to a set as well? On the other hand, it makes the def of $\alpha(\vecv)$ trickier... I will leave it up to you, but note that whenever you ``abuse'' notations for the first time, you gotta mention it.}
    corresponds to exactly one clause $C\in \cC$, let $\alpha : V \to \{ 0, 1 \}$ be an arbitrary satisfying assignment. Our algorithm proceeds in rounds, and each round makes $\poly(n)$ guesses about $\alpha$. Ideally, one of the guesses will allow us to correctly identify the $\alpha$ values for $\Omega(n)$ variables so that the recursion will yield a quasi-polynomial time algorithm.
    
    
    In the case where all $\poly(n)$ guesses fail, we can produce a complete \ncsp{(k-1)} instance which is guaranteed to satisfy by $\alpha$. Thus, it suffices to enumerate all the \ncsp{(k-1)} solutions for the produced instance and see whether they are good for the original \kcsp. 


    We inductively assume that we have the enumeration algorithm for \ncsp{(k-1)}, and we now present our main subroutine for \kcsp. Note that the base case for \ncsp{2} follows from \Cref{cor:2satassgn}.
    
    \paragraph{Overview.}
    Let $\alpha : V \to \{ 0, 1 \}$ be one of the satisfying assignments we are interested in. 
    Consider a $(k-1)$-tuple of variables $\vecv \in \binom{V}{k-1}$. Then, every clause $C =(\vecv, u)$--- out of the total $n-k+1$ clauses containing the $(k-1)$-tuple --- such that $P_C(\alpha^*(\vecv), \alpha')=\sat$ if and only if $\alpha'=\alpha(u)$, must fix the $k$'th literal to $\alpha(u)$. We define this formally as follows:
    % The idea is to guess every optimal assignment to  $k-1$ ``good'' variables that fix the assignment to $\Omega(n)$ other variables. Then, recurse on the smaller (still complete) instance. Note that by every optimal assignment to some variables, say $V'$, we mean every satisfying assignment to $V'$ that is a part of some satisfying assignment of the entire instance, if the instance is satisfiable. Otherwise, if the instance is not satisfiable, we try out all the possibilities and end up with an empty set of satisfying assignments for the entire instance.

    
   % For a $(k-1)$-tuples of variables $\vecv \in V^{k-1}$, assume that the we guess the optimal assignment to be $\alpha(\vecv)\in\{0,1\}^{k-1}$. Given the assignment $\alpha(\vecv)$, we call a clause $(\vecv, v)$ a \emph{fixed clause} (for all $v\in V\setminus \vecv$, that totals to $(n-k+1)$ clauses containing the $(k-1)$-tuple) if the predicate $P_{(\vecv, v)}(\alpha(\vecv),\alpha(v))$ is satisfied only for one assignment $\alpha(v)\in\{0,1\}$ to the $k$'th variable $v$. Let's call this $k$'th variable a \emph{fixed variable}. We define the number of such variables $n_{\vecv, \alpha(\vecv)}$ for the given tuple $\vecv$ and assignment $\alpha(\vecv)$ below.
    % \begin{definition}[Induced Predicate]\label{def:induced predicate}
    %     Given any clause $C$, any subset $V\subset C$ of variables, and any assignment $\alpha(V)$. We define $P^{\alpha(V)}_C:\Sigma^{|C\setminus V|}\mapsto \{\sat,\unsat\}$ as the induced predicate given the partial assignment $\alpha(V)$ to variables $V$ of $C$ such that $P^{\alpha(V)}_C(\alpha(C\setminus V))=P_C(\alpha(V),\alpha(C\setminus V))$  for all possible values of $\alpha(C\setminus V)\in \{0,1\}^{|C\setminus V|}$.
    % \end{definition}
    \begin{definition}[Fixed Variables]\label{def:kcspmaj}
        Given a \ncsp{k} instance, any $(k-1)$-tuple of variables $\vecv\in \binom{V}{k-1}$ and any possible assignment of $\alpha(\vecv)\in\{0,1\}^{k-1}$. We define the set of fixed variables as $N_{\vecv,\alpha(\vecv)}=\{v \in V \setminus \vecv \ |\ P_C(\alpha(\vecv), \alpha'(u))=\sat \mbox{ exactly for one value of } \alpha'(u)\in\{0,1\},\ \mbox{ where } C=(\vecv,u)\}$ 
        and the number of fixed variables as $n_{\vecv,\alpha(\vecv)}=|N_{\vecv,\alpha(\vecv)}|$. Moreover, define the corresponding unique assignment as $\alpha_{\vecv,\alpha(\vecv)}(N_{\vecv,\alpha(\vecv)})$.
    \end{definition}

    Call $\vecv\in \binom{V}{k-1}$ a \emph{good $(k-1)$-tuple  with respect to $\alpha$} if the value $n_{\vecv, \alpha(\vecv)}\geq \eps_k n$. So guessing the values $\alpha(\vecv)$ correctly (w.r.t. $\alpha$), fixes at least $\eps_k n$ variables. If we can iterate this process for $\frac{\log n}{\eps_k}$ iterations, we will fix all variables and find $\alpha$. 
    
    
    Now, consider the case where for every $(k-1)$-tuple $\vecv$, we have $n_{\vecv, \alpha(\vecv)} < \eps_k n$. Thus, $\veca' := \arg \max_{\veca\in\{0,1\}^{k-1}} n_{\vecv, \veca}$ can not be the same as $\alpha(\vecv)$ (for any constant $\eps_k \leq \frac{1}{2^{k+1}})$. We add a \ncsp{(k-1)} constraint $P_\vecv(\alpha''(\vecv))=\unsat$ if and only if $\alpha''(\vecv)=\veca'$, which is surely satisfied by $\alpha$. Doing the same for all $(k-1)$-tuples, we get a complete \ncsp{(k-1)} instance. From \Cref{lem:satnumberassgn}, we know that the number of satisfiable assignments for a complete \ncsp{(k-1)} instance on $n$ variables can be at most $O(n^{k-1})$, and using our induction hypothesis, these can be computed in time $n^{O(\log n)}$. Thus, we can enumerate all the satisfying assignments to the created \ncsp{(k-1)} instance, and $\alpha$ will be one of them. 

    % \paragraph{Intuition.} Let's call the $(k-1)$-tuple $\vecv$ and the optimal assignment $\alpha^*(\vecv)$ a \emph{good $(k-1)$-tuple} if for some optimal assignment the number of fixed variables $n_{\vecv,\alpha^*(\veca)}$ is at least $\eps_kn$. If there is a good tuple $\vecv, \alpha^*(\vecv)$ in the instance, then we can guess the tuple and its optimal assignment $\alpha^*(\vecv)$ in time $2^{k-1}\cdot\binom{n}{k-1} = n^{O(k)}$. Then we can fix at least a constant fraction $\eps_kn$ of fixed variables defined by the set $N_{\vecv,\alpha^*(\veca)}$. We can forget about the fixed variables then and try to recursively solve the problem of \ncsp{k} on the un-fixed variables that are at most $(1-\eps_k)n$ many. Note that, there could still be constraints between fixed and un-fixed variables. However, we claim to enumerate all possible satisfying assignments for the un-fixed variables, and we check all of them for the satisfiability of the whole instance.

    % The other case is when there are no such good $(k-1)$-tuples. Then, it is safe to assume that $n_{\vecv,\alpha^*(\vecv)}<\eps_kn$ for all optimal assignments $\alpha^*(\vecv)$. Since the instance is a complete instance, we have that the sum of $n_{\vecv,\alpha(vecv)}$ over all the $\alpha(\vecv)\in\{0,1\}^{|\vecv|}$ is exactly $n-k+1$. Thus, for large enough $n$ ($n>2k-1$, otherwise we can just brute force), and any constant $k$ and any $0<\eps<\frac{1}{2^{k+1}}$, we must have that $\alpha'(\vecv)=\arg\max_{\alpha(\vecv)\in\{0,1\}^{|\vecv|}}n_{\vecv,\alpha(\vecv)}$ (breaking ties arbitrarily) does not correspond to any of the optimal assignments $\alpha^*(\vecv)$ as the maximum value must be at least $\frac{n}{2^{k}}$ by simple averaging argument. We can therefore add the \ncsp{(k-1)} constraint $C=\vecv$ such that $P_C(\alpha(\vecv))=\unsat$ iff $\alpha(\vecv)=\alpha'(\vecv)$. Since we add these \ncsp{(k-1)} constraints for every pair, we claim that the instance is a complete \ncsp{(k-1)} instance. Using induction, we have an algorithm that decides the satisfiability of a complete \ncsp{(k-1)} instance as well as outputs all the satisfiable assignments to it in time $n^{O({\log n})}$.

     \paragraph{Algorithm.} The \Cref{alg:kcspassgn} takes in input as the variables $V$, the complete instance clauses $\cC$, and an partial assignment to all the literals $\alpha:V\mapsto\{0,1,\frac12\}$ where for any undecided variable $v$, $\alpha(v) = \frac12$. Initially, the assignment $\alpha$ is completely undecided, i.e., $\alpha(v)=\frac12$ for all $v\in V$. It outputs $\cA$, which will eventually be all satisfying assignments to $(V, \cC)$. 


    The algorithm first computes the set of unfixed variables $V_U = \{v\in V\ |\ \alpha(v) = \frac12\}$. In Step \ref{algkcspassgnstep:lessvars}, if there are only $O(\log n)$ unfixed variables, we enumerate all assignments and check whether they give a satisfying assignment. This takes time $2^{|V_U|} \cdot \poly(n) = \poly(n)$.
        

    The algorithm branches by either guessing one of the good $(k-1)$-tuples (Step \ref{algkcspassgnstep:guess}) and their assignment, or assuming that there are no good $(k-1)$-tuples, forms a complete \ncsp{(k-1)} instance (Step \ref{algkcspassgnstep:2sat}). 
    
    
    In Step \ref{algkcspassgnstep:guess}, we guess a $(k-1)$-tuple $\vecv\in\binom{V_U}{k-1}$ by branching over all $(k-1)$-tuples of unfixed variables and guess their optimal assignment $\veca$. If the guessed $(k-1)$-tuple is a good $(k-1)$-tuple with respect to some satisfying assignment $\alpha$, i.e., if $n_{\vecv, \alpha(\vecv)}\geq \eps_k|V_U|$, then we can correctly fix at least $\eps_k |V_U|$ variables $N_{\vecv, \alpha(\vecv)}$ and solve the problem recursively. Thus we only need to recurse to depth at most $\frac{\log n}{\eps_k}$ before fixing all the variables optimally. This is ensured by Step \ref{algkcspassgnstep:depth}. 


    In Step \ref{algkcspassgnstep:2sat}, we branch by assuming that there is no good $(k-1)$-tuple with respect to $\alpha$ among the unfixed variables. Under this assumption, we know that $n_{\vecv, \alpha(\vecv)}< \eps_k| V_U|$. Since, all the $2^{k-1}$ quantities $n_{\vecv, \veca}$ over all $\veca\in\{0,1\}^{k-1}$ sum up to at least $|V_U|-k+1$ as there is at least one unsatisfying assignment for each clause. Defining $\veca' := \mathrm{argmax}_{\veca\in\{0,1\}^{k-1}}n_{\vecv, \veca}$ (while arbitrarily breaking ties) ensures that $\alpha(\vecv) \neq \veca'$ for any $\eps_k \leq \frac{1}{2^{k+1}}$. 
    So, we add the \ncsp{(k-1)} constraints $P_\vecv(\alpha''(\vecv))=\unsat$ if and only if $\alpha''(\vecv)=\veca'$, for all $\vecv\in \binom{V_U}{k-1}$. This gives us a complete \ncsp{(k-1)} instance $\cC_{k-1}$ over the unfixed variables that is guaranteed to be satisfied by $\alpha$. In Steps \ref{algkcspassgnstep:find2sat} and \ref{algkcspassgnstep:check2sat}, we compute and check whether any of the satisfiable assignments of the \ncsp{(k-1)} instance $\cC_{k-1}$ satisfy the \ncsp{k} instance $\cC$ or not. We add every such satisfying assignment to the set $\cA$.

    % \paragraph{Algorithm. }  The \Cref{alg:kcspassgn} takes in input as the variables $V$, the complete instance clauses $\cC$, and a partial assignment to all the variables $\alpha:V\mapsto[0,1,\frac12]$. For any variable $v$, if the assignment is undecided $\alpha(v) = \frac12$.  Initially, the assignment $\alpha$ is completely undecided, i.e., $\alpha(v)=\frac12$ for all $v\in V$.

    
    %     In Step \ref{algkcspassgnstep:lessvars}, we first directly guess all the possible optimal assignments of the unfixed variables if there are only $O(\log n)$ many of them. This takes time $2^{|V_U|} = \poly(n)$. Then, in another $\poly(n)$, we check whether each of the whole assignments satisfies all the clauses of the $\ncsp{k}$ instance. If yes, we add the assignment $\alpha$ to the set of all satisfying assignments $\cA$.
    
    %     The algorithm branches by either guessing all the good $(k-1)$-tuples (one in each branch)(Step \ref{algkcspassgnstep:guess}), or assuming that there are no good tuples and forms a complete $\ncsp{(k-1)}$ instance (Step \ref{algksatassgnstep:2sat}). For every branch that returns that there is a satisfying assignment, we conclude that the instance is satisfiable and add the assignment to $\cA$. Otherwise, if none of the branches return that there is a satisfiable assignment, then we conclude that the instance is unsatisfiable. 
        
        
    %     In Step \ref{algkcspassgnstep:guess}, we guess a $(k-1)$-tuple $\vecv,\alpha(\vecv)$ by branching over all pairs of unfixed variables and all their optimal assignment. We only branch, if the guessed-tuple if $n_{\vecv, \alpha(\vecv)}\geq \eps|V_U|$, then we fix at least $\eps|V_U|$ variables to $\alpha_{\vecv, \alpha(\vecv)}(N_{\vecv, \alpha(\vecv)})$ and solve the problem recursively. We only recurse to a depth at most $\frac{10}{\eps_k}\log n$. This is ensured by Step \ref{algkcspassgnstep:depth}. 
        
        
    %     In Step \ref{algkcspassgnstep:2sat}, we branch by assuming that there is no good $(k-1)$-tuple among the unfixed variables. We add the (\ncsp{(k-1)}) constraint that the $(k-1)$-tuple $\vecv$ can not be assigned $\alpha'(\vecv)$ that maximizes $\max_{\alpha(\vecv)\in\{0,1\}^{k-1}}n_{\vecv,\alpha(\vecv)}$ (while arbitrarily breaking ties). We add the \ncsp{(k-1)} constraint $C=\vecv$ such that $P_C(\alpha(\vecv))=\unsat$ iff $\alpha(\vecv)=\alpha'(\vecv)$. Since we add these \ncsp{(k-1)} constraints for every pair in $V_U$, we later claim that the instance is a complete \ncsp{(k-1)} instance. Using induction, we have an algorithm that decides the satisfiability of a complete \ncsp{(k-1)} instance as well as outputs all the satisfiable assignments to it in time $n^{O({\log n})}$. In Steps \ref{algkcspassgnstep:find2sat} and \ref{algkcspassgnstep:check2sat}, we compute and check whether all the satisfiable assignments of the $\ncsp{(k-1)}$ instance $\cC_{k-1}$ satisfy the $\ncsp{k}$ instance $\cC$ or not. We add every such satisfying assignment to the set $\cA$.

    
        \begin{algorithm}[!htb]
            \caption{ALG-$\kcsp$-decision$_{\cA}(V,\cC,\alpha, d)$}
            \label{alg:kcspassgn}
            \begin{algorithmic}[1]
                \Require $V, \cC, \alpha:V\mapsto \{\frac12, 1, 0\}, d$
                % \State $\mathrm{ret}\gets 0$ \Comment{Value to return, $0$ if unsatisfied, and $1$ otherwise}
                \IIf{$d>\frac{10}{\eps_k} \log |V|$} \label{algkcspassgnstep:depth}
                    \Return %$\mathrm{ret}$ \Comment{If depth exceeds $O(\log n)$, return $0$}
                \EndIIf
                \State $V_U \gets \{v\ |\ \alpha(v)\neq\frac12, \forall v\in V\}$ and $V_F \gets V\setminus V_U$\label{algkcspassgnstep:unfix1}
                \Comment{unfixed and fixed variables}
                % \State $\cC_U \gets \{C\ | C\cap V_F= \emptyset, \forall c\in \cC\}$\Comment{complete instance induced on unfixed variables}\label{algkcspassgnstep:unfix2}
                \If{$|V_U|\leq 100 \log n$} \label{algkcspassgnstep:lessvars}
                    % \For{all $\alpha(V_U)\in\{0,1\}^{|V_U|}$}\Comment{Guess optimal assignment $\alpha(V_U)$ of all variables in $V_U$.}
                    %     \If{check-assignment($V, \cC, \alpha)=1$}
                    %         \State $\mathrm{ret}\gets 1$.
                    %         \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    %     \EndIf
                    % \EndFor
                    \State For each assignment to $\alpha : V_U \to \{ 0, 1\}$, if the entire $\alpha$ satisfies $\calC$, add $\alpha$ to $\cA$. 
                \EndIf
                \For{all $\vecv\in V_U^{k-1} $}\label{algkcspassgnstep:guess}\Comment{Guess a $(k-1)$-tuple}
                    \For{all $\veca\in \{0,1\}^{k-1}$}\Comment{Guess the optimal assignment}
                        \If{$n_{\vecv,\veca} \geq \eps_k|V_U|$}
                            \State Let $\alpha'$ be the extension of $\alpha$ where $\alpha'(\vecv)\gets \veca$ and 
                            \State Set $\alpha'(N_{\vecv, \veca})\gets \alpha_{\vecv, \veca}(N_{\vecv, \veca})$. \Comment{Assign all fixed variables}
                            \State ALG-$\ncsp{k}$-decision$_{\cA}(V, \cC, \alpha', d+1)$.\Comment{Recurse}
                            % \State $\alpha(\vecv, N_{\vecv, \alpha(\vecv)})\gets\frac12$.
                        \EndIf
                    \EndFor
                \EndFor
                \State $\cC_{k-1}\gets \emptyset$ \Comment{Set of \ncsp{(k-1)} constraints} 
                \For{all $\vecv\in V_U^{k-1} $}\label{algkcspassgnstep:2sat}\Comment{If no good tuple, add \ncsp{(k-1)} constraints}
                    \State $\veca' \gets \arg\max_{\veca\in \{0,1\}^{k-1} }n_{\vecv, \veca}$ \Comment{Find the maximum fixing value}
                    \State Create \ncsp{(k-1)} constraint $C=\vecv$ such that $P_C(\alpha(\vecv))=\unsat$ iff $\alpha(\vecv)=\veca'$.
                    \State $\cC_{k-1}\gets \cC_{k-1}\cup \{C\}$
                \EndFor
                \State Compute $\cA(V_U, \cC_{k-1})$. \label{algkcspassgnstep:find2sat}\Comment{Compute all the satisfiable assignments of the complete \ncsp{(k-1)} instance}
                \For{$\alpha(V_U) \in \cA(V_U,\cC_{k-1})$}\label{algkcspassgnstep:check2sat}\Comment{Enumerate over all satisfiable complete \ncsp{(k-1)} assignments}
            
                    \If{check-assignment($V,\cC,\alpha) =1$}
                        % \State $\mathrm{ret}\gets 1$.
                        \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    \EndIf \Comment{Return $1$ if some branch finds a satisfiable assignment}
                    % \State $\alpha(V_U)\gets\frac12$.
                \EndFor
                % \State Remove-duplicates$(\cA)$.
                % \State \Return $\mathrm{ret}$. \Comment{Return $0$ if none of the branches find a satisfiable assignment}
            \end{algorithmic}
        \end{algorithm}

        \paragraph{Correctness.} For the correctness of the algorithm, we need to prove that the algorithm outputs the set of all the satisfying assignments to the instance.
        We now prove that the set of satisfying assignments $\cA$ of the algorithm contains all the satisfying assignments to the instance.
    
        \begin{lemma}\label{lem:kcspallassgn}
            Every satisfying assignment $\alpha^*$ belongs to $\cA$.
        \end{lemma}
        \begin{proof}
            Consider any satisfying assignment $\alpha^*$. We prove that in each recursive call, 
            (Case 1) if there exists a good $(k-1)$-tuple $\vecv$ with respect to $\alpha^*$, we will correctly fix at least $ \eps_k|V_U|$ values of $\alpha^*$ in one of the branches, and 
            (Case 2) if there is no good $(k-1)$-tuple, we create a complete \ncsp{(k-1)} instance satisfied by $\alpha^*$. 
            If this is true, then in at most $ \frac{\log n}{\eps_k}$ recursive depth, we would end up guessing $\alpha^*$ in at least one leaf and return $1$ and store $\alpha^*$ in $\cA$.
            
            \paragraph{Case 1: Branching over good-$(k-1)$-tuples:} Suppose that for some $(k-1)$-tuple $\vecv\in\binom{V_U}{k-1}$ is good $(k-1)$-tuple w.r.t $\alpha^*$; i.e., $n_{\vecv, \alpha^*(\vecv)} \geq \eps_k|V_U|$. Then the algorithm would branch over this choice of $\vecv, \alpha^*(\vecv)$ as it branches over all the possible choices of good $(k-1)$-tuples. Then, the algorithm sets $\alpha^*(\vecv)$ as well as $\alpha^*(N_{\vecv, \alpha^*(\vecv)})$ correctly (follows from the \Cref{def:kcspmaj} of fixed variables). 
            
            
            \paragraph{Case 2: Branching over complete \ncsp{(k-1)}:} If in a recursive call of the algorithm, for no $(k-1)$-tuple $\vecv\in \binom{V_U}{k-1}$, we have that $n_{\vecv,\alpha^*(\vecv)} \geq \eps_k|V_U|$, then consider the branch where the algorithm forms a complete \ncsp{(k-1)} on the unfixed variables $V_U$ in Step \ref{algkcspassgnstep:2sat}. 
            (Note that the $(k-1)$-tuple $\vecv$ can still be a good $(k-1)$-tuple w.r.t. some other optimal assignment $\alpha^{**}$.)
            We claim that the complete \ncsp{(k-1)} instance is satisfiable by assignment $\alpha^*(V_U)$, which is the restriction of $\alpha^*$ to $V_U$. 

    
            If this were true, then we would be done as we branch over all the possible \ncsp{(k-1)} assignments to $V_U$, and $\alpha^*(V_U)$ must be one of them. 
            
            Fix any $(k-1)$-tuple $\vecv\in \binom{V_U}{k-1}$. 
            We know that $n_{\vecv, \alpha^*(\vecv)}< \eps_k|V_U|$. 
            Since, all the $2^{k-1}$ quantities $n_{\vecv,\alpha(\vecv)}$, over all $\alpha(\vecv)\in\{0,1\}^{k-1}$, sum up to at least $|V_U|-k+1$ (as every clause has at least one unsatisfying assignment), the $\max_{\alpha(\vecv)\in\{0,1\}^{3}}n_{\vecv,\alpha(\vecv)}$ must be at least $\frac{|V_U|-k+1}{2^{k-1}}\geq\frac{|V_U|}{2^k}$ (as $|V_U|>\Omega(\log n)$, and $n$ is large enough) by averaging argument. This maximum value does not correspond to the $n_{\vecv, \alpha^*(\vecv)}$ value for any $\eps_k \leq \frac{1}{2{k+1}}$. Since this $(k-1)$-tuple $\alpha(\vecv)$ that achieves the maximum is exactly what our added \ncsp{(k-1)} constraint rules out, $\alpha^*(\vecv)$ will satisfy this constraint. 
        \end{proof} 
    
       
        

    \paragraph{Analysis.} The algorithm either branches over all the $2^{k-1}\cdot \binom{|V_U|}{k-1}$ number of guesses of $(k-1)$-tuples and their assignments, or formulates the complete \ncsp{(k-1)} instance $\cC_{k-1}$ on $V_U$, and checks whether any \ncsp{(k-1)} assignment satisfies the \ncsp{k} instance $\cC$ or not. Since, the former fixes at least $\eps_k |V_U|$ variables, the depth of the branching tree would be at most $\frac{\log n}{\eps_k}$ before we can correctly arrive at a conclusion. For the latter, \aay{using our induction hypothesis}, we know that all the assignments to $V_U$ satisfying the \ncsp{(k-1)} instance $\cC_{k-1}$ can be found in $n^{O(\log n)}$ time (this bounds the number of assignments as well).
    Since there are at most $(2^{k-1}n^{k-1})^{\frac{\log n}{\eps_k}}$ recursive calls and each call takes $n^{O(\log n)}$ time, the total runtime of the algorithm is $n^{O(\log n)} \cdot (2^{k-1}n^{k-1})^{\frac{\log n}{\eps_k}} = n^{O(\log n)}$, for $\eps_k=\frac{1}{2^{k+1}}$ and any constant $k$ which yields the following theorem. 
    

    % \paragraph{Correctness.} For the correctness of the algorithm, we need to prove that the algorithm outputs the set of all the satisfying assignments to the instance (an empty set if and only if the instance is unsatisfiable). 
    

    %     \begin{lemma}\label{lem:kcspsat}
    %         Every assignment $\alpha(V)\in\cA$ is a satisfying assignment.
    %     \end{lemma}
    %     \begin{proof}
    %         This is trivial to prove as before adding an assignment to $\cA$ (in Steps \ref{algkcspassgnstep:lessvars}, \ref{algkcspassgnstep:check2sat}), we check whether the assignment satisfies the entire instance or not.
    %     \end{proof}
    %     We now prove that the set of satisfying assignments $\cA$ of the algorithm contains all the satisfying assignments to the instance.
    
    %     \begin{lemma}\label{lem:kcspallassgn}
    %         Every satisfying assignment $\alpha^*$ belongs to $\cA$.
    %     \end{lemma}
    %     \begin{proof}
    %         The proof is similar to that of $\kcsp$ (\Cref{lem:4satallassgn}). 
    %         Consider any satisfying assignment $\alpha^*$. We prove that in each recursive call we guess at least $\eps |V_U|$ values of $\alpha^*$ in one of the branches. If this is true, then in $\frac{2}{\eps_k} \log n$ calls, we would end up guessing $\alpha^*$ in at least one leaf and return $1$ and store $\alpha^*$ in $\cA$.
            
            
    %         \paragraph{Case 1: Branching over complete \ncsp{(k-1)}:} If in a recursive call of the algorithm, for all for all $\vecv\in V_U^{k-1}$, we have $n_{\vecv, \alpha^*(\vecv)}< \eps_k|V_U|$. Then we form a complete $\ncsp{(k-1)}$ on the unfixed variables $V_U$ as in Step \ref{algkcspassgnstep:2sat}. 
    %         We claim that the complete \ncsp{(k-1)} instance is satisfiable by assignment $\alpha^*(V_U)$ (given $\alpha^*$ is an optimal assignment). If this were true, then we would be done as we branch over all the possible \ncsp{(k-1)} assignments to $V_U$, and $\alpha^*(V_U)$ must be one of them. 
            
    %         So, for all for all $\vecv\in V_U^{k-1}$, we have $n_{\vecv, \alpha^*(\vecv)}< \eps_k|V_U|$. Since, all the $2^{k-1}$ quantities $n_{\vecv,\alpha(\vecv)}$, over all $\alpha(\vecv)\in\{0,1\}^{k-1}$, sum up to $|V_U|-k+1$, the $\max_{\alpha(\vecv)\in\{0,1\}^{k-1}}n_{\vecv,\alpha(\vecv)}$ must be at least $\frac{1}{2^{k}}|V_U|$ by averaging argument. Thus, for any $\eps_k <\frac{1}{2^{k}}$, this maximum value can not correspond to the $n_{\vecv, \alpha^*(\vecv)}$ value. This is exactly the constraint that we add to the $\ncsp{(k-1)}$ clause in the algorithm. Thus, it is clear that each \ncsp{(k-1)} constraint is satisfied by $\alpha^*$ as $\alpha^*(\vecv)\neq \alpha'(\vecv)$ that maximizes $\max_{\alpha(\vecv)\in\{0,1\}^{k-1}}n_{\vecv,\alpha(\vecv)}$. 
    %         Thus, we get $\alpha^*(\vecv)$ correctly if we enumerate all the satisfying assignments of the complete instance.
            
            
            
            
    %         \paragraph{Case 2: Branching over good tuples:} Else if for some $(k-1)$-tuples $\vecv$, we have that $\vecv, \alpha^*(\vecv)$ is a good $(k-1)$-tuple w.r.t $\alpha^*$, i.e., $n_{\vecv, \alpha^*(\vecv)}< \eps_k|V_U|$. Then the algorithm would branch over this choice of $\vecv$ as it branches over all the possible choices of good tuples. Then, the algorithm guessed $\alpha^*(\vecv)$ and sets $\alpha^*(N_{\vecv, \alpha^*(\vecv)})$ correctly in on of the branches (follows from the \Cref{def:kcspmaj} of fixed variables). %The number of such recursive calls is at most $\frac{2}{\eps_k}\log n$ as we fix $\eps_k$ fraction of variables each time. Thus, the algorithm would correctly return $1$ and store the exact assignment $\alpha^*$ in $\cA$ at the end.
    %     \end{proof} 


    % \paragraph{Analysis.} The algorithm either branches over all the $|V_U|^{O(k)}$ number of guesses of pairs, or formulates the complete $\ncsp{(k-1)}$ instance $\cC_{k-1}$ on $V_U$, and checks whether any $\ncsp{(k-1)}$ assignment satisfies the $\ncsp{(k-1)}$ instance $\cC$ or not. Since, the former fixes at least $\eps_k|V_U|$ variables, the depth of the branching tree would be at most $\frac{1}{\eps_k}\log n$ before we can correctly arrive at a conclusion. Fix $\eps_k = \frac{1}{2^{k+1}}$. For the latter, we use induction to establish that all the assignments to $V_U$ satisfying the complete $\ncsp{(k-1)}$ instance $\cC_{k-1}$ can be found in $n^{O(\log n)}$ time (the number of assignments is bounded by $O(n^{k-1})$ from \Cref{lem:satnumberassgn}). This also gives us that $|\cA|$ before we remove duplicates can be at most the number of leaves in the recursion tree, i.e., $n^{O(\log n)}$. From \Cref{lem:satnumberassgn}, we know that the total number of satisfiable assignments (i.e., the total size of $\cA$ after removing duplicates) is at most $O(n^{k-1})$.
        
    
  
    \begin{theorem}\label{thm:kcspassgn}
        For any constant $k$, there is a $n^{O(\log n)}$ time algorithm to decide whether a complete instance of $\kcsp$ on $n$ variables is satisfiable or not. Moreover, this algorithm also returns all the satisfying assignments.
    \end{theorem}



==> Inputs/kcsp.tex <==
\section{$k$-CSP}
\label{sec:kcsp}
In this section, we present a quasi-polynomial algorithm for complete $k$-CSP, proving Theorem~\ref{thm:kcsp}; again, in addition to deciding the satisfiability of the instance, our algorithm enumerates all the satisfying assignments. 
    Given an instance $(V, \calC)$ where each $k$-tuple of variables $V_k \in \binom{V}{k}$
    %\euiwoong{$\binom{V}{k}$ is the collection of $k$-sets. Given $C$ is a technically a set as well, it makes sense to change $\vecv$ to a set as well? On the other hand, it makes the def of $\alpha(\vecv)$ trickier... I will leave it up to you, but note that whenever you ``abuse'' notations for the first time, you gotta mention it.}
    corresponds to exactly one clause $C\in \cC$, let $\alpha : V \to \{ 0, 1 \}$ be an arbitrary satisfying assignment. Our algorithm proceeds in rounds, and each round makes $\poly(n)$ guesses about $\alpha$. Ideally, one of the guesses will allow us to correctly identify the $\alpha$ values for $\Omega(n)$ variables so that the recursion will yield a quasi-polynomial time algorithm.
    
    
    In the case where all $\poly(n)$ guesses fail, we can produce a complete \ncsp{(k-1)} instance which is guaranteed to satisfy by $\alpha$. Thus, it suffices to enumerate all the \ncsp{(k-1)} solutions for the produced instance and see whether they are good for the original \kcsp. 


    We inductively assume that we have the enumeration algorithm for \ncsp{(k-1)}, and we now present our main subroutine for \kcsp. Note that the base case for \ncsp{2} follows from \Cref{cor:2satassgn}.
    
    \paragraph{Overview.}
    Let $\alpha : V \to \{ 0, 1 \}$ be one of the satisfying assignments we are interested in. 
    Consider a $(k-1)$-tuple of variables $V_{k-1} \in \binom{V}{k-1}$. Then, every clause $C =(V_{k-1}, u)$--- out of the total $n-k+1$ clauses containing the $(k-1)$-tuple --- such that \aay{$P_C(\alpha((V_{k-1},v)))=\sat$ for exactly one value of $\alpha(v)$, must fix the $k$'th literal to $\alpha(v)$.} We define this formally as follows:
    \aayr{is it fine to write $C=(V_{k-1}, u)$? Or should we write it as $C=V_{k-1}\cup\{u\}$?}
    
    
    \begin{definition}[Fixed Variables]\label{def:kcspmaj}
        Given a \ncsp{k} instance, any $(k-1)$-tuple of variables $V_{k-1}\in \binom{V}{k-1}$ and any possible assignment of $\alpha_{V_{k-1}}\in\{0,1\}^{k-1}$. We define the set of \aay{fixed variables as $N_{V_{k-1},\alpha(V_{k-1})}=\{v \in V \setminus V_{k-1} \ |\ P_C(\alpha((V_{k-1},u))=\sat$ exactly for one value of $\alpha'_u\in\{0,1\},$ where $\alpha(V_{k-1})=\alpha_{V_{k-1}}, \alpha(u)=\alpha_u, C=(V_{k-1},u)\}$ 
        and the number of fixed variables as $n_{V_{k-1},\alpha(V_{k-1})}=|N_{V_{k-1},\alpha(V_{k-1})}|$. Moreover, define the corresponding unique assignment as $\alpha_{V_{k-1},\alpha(V_{k-1})}(N_{V_{k-1},\alpha(V_{k-1})})$.}
    \end{definition}
    \euiwoong{Pedantically again, the application of $P_C$ is order-sensitive unless it is given a set (which was mentioned in the intro).}

    Call $V_{k-1}\in \binom{V}{k-1}$ a \emph{good $(k-1)$-tuple  with respect to $\alpha$} if the value $n_{V_{k-1}, \alpha(V_{k-1})}\geq \eps_k n$. So guessing the values $\alpha(V_{k-1})$ correctly (w.r.t. $\alpha$), fixes at least $\eps_k n$ variables. If we can iterate this process for $\frac{\log n}{\eps_k}$ iterations, we will fix all variables and find $\alpha$. 
    
    
    Now, consider the case where for every $(k-1)$-tuple $V_{k-1}$, we have $n_{V_{k-1}, \alpha(V_{k-1})} < \eps_k n$. Thus, $\alpha_{V_{k-1}}' := \arg \max_{\alpha_{V_{k-1}}\in\{0,1\}^{k-1}} n_{V_{k-1}, \alpha_{V_{k-1}}}$ can not be the same as $\alpha(V_{k-1})$ (for any constant $\eps_k \leq \frac{1}{2^{k+1}})$. We add a \ncsp{(k-1)} constraint $P_{V_{k-1}}(\alpha''(V_{k-1}))=\unsat$ if and only if $\alpha''(V_{k-1})=\alpha_{V_{k-1}}'$, which is surely satisfied by $\alpha$. Doing the same for all $(k-1)$-tuples, we get a complete \ncsp{(k-1)} instance. From \Cref{lem:satnumberassgn}, we know that the number of satisfiable assignments for a complete \ncsp{(k-1)} instance on $n$ variables can be at most $O(n^{k-1})$, and using our induction hypothesis, these can be computed in time $n^{O(\log n)}$. Thus, we can enumerate all the satisfying assignments to the created \ncsp{(k-1)} instance, and $\alpha$ will be one of them. 

   
    

     \paragraph{Algorithm.} The \Cref{alg:kcspassgn} takes in input as the variables $V$, the complete instance clauses $\cC$, and an partial assignment to all the literals $\alpha:V\mapsto\{0,1,\frac12\}$ where for any undecided variable $v$, $\alpha(v) = \frac12$. Initially, the assignment $\alpha$ is completely undecided, i.e., $\alpha(v)=\frac12$ for all $v\in V$. It outputs $\cA$, which will eventually be all satisfying assignments to $(V, \cC)$. 


    The algorithm first computes the set of unfixed variables $V_U = \{v\in V\ |\ \alpha(v) = \frac12\}$. In Step \ref{algkcspassgnstep:lessvars}, if there are only $O(\log n)$ unfixed variables, we enumerate all assignments and check whether they give a satisfying assignment. This takes time $2^{|V_U|} \cdot \poly(n) = \poly(n)$.
        

    The algorithm branches by either guessing one of the good $(k-1)$-tuples (Step \ref{algkcspassgnstep:guess}) and their assignment, or assuming that there are no good $(k-1)$-tuples, forms a complete \ncsp{(k-1)} instance (Step \ref{algkcspassgnstep:2sat}). 
    
    
    In Step \ref{algkcspassgnstep:guess}, we guess a $(k-1)$-tuple $V_{k-1}\in\binom{V_U}{k-1}$ by branching over all $(k-1)$-tuples of unfixed variables and guess their optimal assignment $\alpha_{V_{k-1}}$. If the guessed $(k-1)$-tuple is a good $(k-1)$-tuple with respect to some satisfying assignment $\alpha$, i.e., if $n_{V_{k-1}, \alpha(V_{k-1})}\geq \eps_k|V_U|$ \aay{(and $\alpha(V_{k-1})=\alpha_{V_{k-1}}$, i.e., the guess $\alpha_{V_{k-1}}$ is correct w.r.t. $\alpha$ on $V_{k-1}$)}, then we can correctly fix at least $\eps_k |V_U|$ variables $N_{V_{k-1}, \alpha(V_{k-1})}$ and solve the problem recursively. Thus we only need to recurse to depth at most $\frac{\log n}{\eps_k}$ before fixing all the variables optimally. \aay{This is ensured by Step \ref{algkcspassgnstep:lessvars} which optimally computes the assignment to $V_U$ once $|V_U|\leq 100 \log n$.}. 


    In Step \ref{algkcspassgnstep:2sat}, we branch by assuming that there is no good $(k-1)$-tuple with respect to $\alpha$ among the unfixed variables. Under this assumption, we know that $n_{V_{k-1}, \alpha(V_{k-1})}< \eps_k| V_U|$. Since, all the $2^{k-1}$ quantities $n_{V_{k-1}, \alpha_{V_{k-1}}}$ over all $\alpha_{V_{k-1}}\in\{0,1\}^{k-1}$ sum up to at least $|V_U|-k+1$ as there is at least one unsatisfying assignment for each clause. Defining $\alpha_{V_{k-1}}' := \mathrm{argmax}_{\alpha_{V_{k-1}}\in\{0,1\}^{k-1}}n_{V_{k-1}, \alpha_{V_{k-1}}}$ (while arbitrarily breaking ties) ensures that $\alpha(V_{k-1}) \neq \alpha_{V_{k-1}}'$ for any $\eps_k \leq \frac{1}{2^{k+1}}$. 
    So, we add the \ncsp{(k-1)} constraints $P_{V_{k-1}}(\alpha''(V_{k-1}))=\unsat$ if and only if $\alpha''(V_{k-1})=\alpha_{V_{k-1}}'$, for all $V_{k-1}\in \binom{V_U}{k-1}$. \aayr{is this $\alpha(V)$ vs $\alpha_V$ business confusing?}This gives us a complete \ncsp{(k-1)} instance $\cC_{k-1}$ over the unfixed variables that is guaranteed to be satisfied by $\alpha$. In Steps \ref{algkcspassgnstep:find2sat} and \ref{algkcspassgnstep:check2sat}, we compute and check whether any of the satisfiable assignments of the \ncsp{(k-1)} instance $\cC_{k-1}$ satisfy the \ncsp{k} instance $\cC$ or not. We add every such satisfying assignment to the set $\cA$.

    
    
        \begin{algorithm}[!htb]
            \caption{ALG-$\kcsp$-decision$_{\cA}(V,\cC,\alpha, d)$}
            \label{alg:kcspassgn}
            \begin{algorithmic}[1]
                \Require $V, \cC, \alpha:V\mapsto \{\frac12, 1, 0\}, d$
                % \State $\mathrm{ret}\gets 0$ \Comment{Value to return, $0$ if unsatisfied, and $1$ otherwise}
                % \IIf{$d>\frac{10}{\eps_k} \log |V|$} \label{algkcspassgnstep:depth}
                    \Return %$\mathrm{ret}$ \Comment{If depth exceeds $O(\log n)$, return $0$}
                \EndIIf
                \State $V_U \gets \{v\ |\ \alpha(v)\neq\frac12, \forall v\in V\}$ and $V_F \gets V\setminus V_U$\label{algkcspassgnstep:unfix1}
                \Comment{unfixed and fixed variables}
                % \State $\cC_U \gets \{C\ | C\cap V_F= \emptyset, \forall c\in \cC\}$\Comment{complete instance induced on unfixed variables}\label{algkcspassgnstep:unfix2}
                \If{$|V_U|\leq 100 \log n$} \label{algkcspassgnstep:lessvars}
                
                    \State For each assignment to $\alpha : V_U \to \{ 0, 1\}$, if the entire $\alpha$ satisfies $\calC$, add $\alpha$ to $\cA$. 
                \EndIf
                \For{all $V_{k-1}\in V_U^{k-1} $}\label{algkcspassgnstep:guess}\Comment{Guess a $(k-1)$-tuple}
                    \For{all $\alpha_{V_{k-1}}\in \{0,1\}^{k-1}$}\Comment{Guess the optimal assignment}
                        \If{$n_{V_{k-1},\alpha_{V_{k-1}}} \geq \eps_k|V_U|$}
                            \State Let $\alpha'$ be the extension of $\alpha$ where $\alpha'(V_{k-1})\gets \alpha_{V_{k-1}}$ and 
                            \State Set $\alpha'(N_{V_{k-1}, \alpha_{V_{k-1}}})\gets \alpha_{V_{k-1}, \alpha_{V_{k-1}}}(N_{V_{k-1}, \alpha_{V_{k-1}}})$. \Comment{Assign all fixed variables}
                            \State ALG-$\ncsp{k}$-decision$_{\cA}(V, \cC, \alpha', d+1)$.\Comment{Recurse}
                            % \State $\alpha(V_{k-1}, N_{V_{k-1}, \alpha(V_{k-1})})\gets\frac12$.
                        \EndIf
                    \EndFor
                \EndFor
                \State $\cC_{k-1}\gets \emptyset$ \Comment{Set of \ncsp{(k-1)} constraints} 
                \For{all $V_{k-1}\in V_U^{k-1} $}\label{algkcspassgnstep:2sat}\Comment{If no good tuple, add \ncsp{(k-1)} constraints}
                    \State $\alpha_{V_{k-1}}' \gets \arg\max_{\alpha_{V_{k-1}}\in \{0,1\}^{k-1} }n_{V_{k-1}, \alpha_{V_{k-1}}}$ \Comment{Find the maximum fixing value}
                    \State Create \ncsp{(k-1)} constraint $C=V_{k-1}$ such that $P_C(\alpha(V_{k-1}))=\unsat$ iff $\alpha(V_{k-1})=\alpha_{V_{k-1}}'$.
                    \State $\cC_{k-1}\gets \cC_{k-1}\cup \{C\}$
                \EndFor
                \State Compute $\cA(V_U, \cC_{k-1})$. \label{algkcspassgnstep:find2sat}\Comment{Compute all the satisfiable assignments of the complete \ncsp{(k-1)} instance}
                \For{$\aay{\alpha_{V_U}} \in \cA(V_U,\cC_{k-1})$}\label{algkcspassgnstep:check2sat}\Comment{Enumerate over all satisfiable complete \ncsp{(k-1)} assignments}
                    \State \aay{Set $\alpha(V_U)\gets \alpha_{V_U}$.}
                    \If{check-assignment($V,\cC,\alpha) =1$}
                        % \State $\mathrm{ret}\gets 1$.
                        \State $\cA\gets \cA \cup \{\alpha\}$.\Comment{Store the satisfying assignment to set}
                    \EndIf \Comment{Return $1$ if some branch finds a satisfiable assignment}
                    % \State $\alpha(V_U)\gets\frac12$.
                \EndFor
                % \State Remove-duplicates$(\cA)$.
                % \State \Return $\mathrm{ret}$. \Comment{Return $0$ if none of the branches find a satisfiable assignment}
            \end{algorithmic}
        \end{algorithm}

        \paragraph{Correctness.} For the correctness of the algorithm, we need to prove that the algorithm outputs the set of all the satisfying assignments to the instance.
        We now prove that the set of satisfying assignments $\cA$ of the algorithm contains all the satisfying assignments to the instance.
    
        \begin{lemma}\label{lem:kcspallassgn}
            Every satisfying assignment $\alpha^*$ belongs to $\cA$.
        \end{lemma}
        \begin{proof}
            Consider any satisfying assignment $\alpha^*$. We prove that in each recursive call, 
            (Case 1) if there exists a good $(k-1)$-tuple $V_{k-1}$ with respect to $\alpha^*$, we will correctly fix at least $ \eps_k|V_U|$ values of $\alpha^*$ in one of the branches, and 
            (Case 2) if there is no good $(k-1)$-tuple, we create a complete \ncsp{(k-1)} instance satisfied by $\alpha^*$. 
            If this is true, then in at most $ \frac{\log n}{\eps_k}$ recursive depth, we would end up guessing $\alpha^*$ in at least one leaf and return $1$ and store $\alpha^*$ in $\cA$.
            
            \paragraph{Case 1: Branching over good-$(k-1)$-tuples:} Suppose that for some $(k-1)$-tuple $V_{k-1}\in\binom{V_U}{k-1}$ is good $(k-1)$-tuple w.r.t $\alpha^*$; i.e., $n_{V_{k-1}, \alpha^*(V_{k-1})} \geq \eps_k|V_U|$. Then the algorithm would branch over this choice of $V_{k-1}, \alpha^*(V_{k-1})$ as it branches over all the possible choices of good $(k-1)$-tuples. Then, the algorithm sets $\alpha^*(V_{k-1})$ as well as $\alpha^*(N_{V_{k-1}, \alpha^*(V_{k-1})})$ correctly (follows from the \Cref{def:kcspmaj} of fixed variables). 
            
            
            \paragraph{Case 2: Branching over complete \ncsp{(k-1)}:} If in a recursive call of the algorithm, for no $(k-1)$-tuple $V_{k-1}\in \binom{V_U}{k-1}$, we have that $n_{V_{k-1},\alpha^*(V_{k-1})} \geq \eps_k|V_U|$, then consider the branch where the algorithm forms a complete \ncsp{(k-1)} on the unfixed variables $V_U$ in Step \ref{algkcspassgnstep:2sat}. 
            (Note that the $(k-1)$-tuple $V_{k-1}$ can still be a good $(k-1)$-tuple w.r.t. some other optimal assignment $\alpha^{**}$.)
            We claim that the complete \ncsp{(k-1)} instance is satisfiable by assignment $\alpha^*(V_U)$, which is the restriction of $\alpha^*$ to $V_U$. 

    
            If this were true, then we would be done as we branch over all the possible \ncsp{(k-1)} assignments to $V_U$, and $\alpha^*(V_U)$ must be one of them. 
            
            Fix any $(k-1)$-tuple $V_{k-1}\in \binom{V_U}{k-1}$. 
            We know that $n_{V_{k-1}, \alpha^*(V_{k-1})}< \eps_k|V_U|$. 
            \aay{Since, all the $2^{k-1}$ quantities $n_{V_{k-1},\alpha_{V_{k-1}}}$, over all $\alpha_{V_{k-1}}\in\{0,1\}^{k-1}$, sum up to at least $|V_U|-k+1$ (as every clause has at least one unsatisfying assignment), the $\max_{\alpha_{V_{k-1}}\in\{0,1\}^{3}}n_{V_{k-1},\alpha_{V_{k-1}}}$} must be at least $\frac{|V_U|-k+1}{2^{k-1}}\geq\frac{|V_U|}{2^k}$ (as $|V_U|>\Omega(\log n)$, and $n$ is large enough) by averaging argument. This maximum value does not correspond to the $n_{V_{k-1}, \alpha^*(V_{k-1})}$ value for any $\eps_k \leq \frac{1}{2{k+1}}$. Since this $(k-1)$-tuple \aay{ $\alpha'_{V_{k-1}}$ }that achieves the maximum is exactly what our added \ncsp{(k-1)} constraint rules out, $\alpha^*(V_{k-1})$ will satisfy this constraint. 
        \end{proof} 
    
       
        

    \paragraph{Analysis.} The algorithm either branches over all the $2^{k-1}\cdot \binom{|V_U|}{k-1}$ number of guesses of $(k-1)$-tuples and their assignments, or formulates the complete \ncsp{(k-1)} instance $\cC_{k-1}$ on $V_U$, and checks whether any \ncsp{(k-1)} assignment satisfies the \ncsp{k} instance $\cC$ or not. %Since, the former fixes at least $\eps_k |V_U|$ variables, the depth of the branching tree would be at most $\frac{\log n}{\eps_k}$ before we can correctly arrive at a conclusion.
    \aay{Since, the former fixes at least $\eps_k |V_U|$ variables, the depth $d$ of the branching tree would be at most $\frac{\log n}{\eps_k}$ before the remaining number of variables $|V_U|\leq (1-\eps_k)^d n$ is less than $100 \log n$ (in which case Step \ref{algkcspassgnstep:lessvars} guesses the entire assignment to $V_U$ optimally). }
    \euiwoong{{\em Correctly arrive at a conclusion} is not precise. Probably a better way to say is $|V_U| \leq n(1-\eps_k)^d$ so that line 3 kicks in until $d \leq \log n/\eps_k$. Actually, this makes line 1 unnecessary. (When you make a change, do the same for 3SAT as well.)}
    \aayr{yes, let's remove step 1}
    For the latter, using our induction hypothesis, we know that all the assignments to $V_U$ satisfying the \ncsp{(k-1)} instance $\cC_{k-1}$ can be found in $n^{O(\log n)}$ time (this bounds the number of assignments as well).
    Since there are at most $(2^{k-1}n^{k-1})^{\frac{\log n}{\eps_k}}$ recursive calls and each call takes $n^{O(\log n)}$ time, the total runtime of the algorithm is $n^{O(\log n)} \cdot (2^{k-1}n^{k-1})^{\frac{\log n}{\eps_k}} = n^{O(\log n)}$, for $\eps_k=\frac{1}{2^{k+1}}$ and any constant $k$ which yields the following theorem. 
    


    \begin{theorem}\label{thm:kcspassgn}
        For any constant $k$, there is a $n^{O(\log n)}$ time algorithm to decide whether a complete instance of $\kcsp$ on $n$ variables is satisfiable or not. Moreover, this algorithm also returns all the satisfying assignments.
    \end{theorem}



==> Inputs/prelim.tex <==
\section{Preliminaries}

Needed?
